The Optimal Decoder is Tilted Temperature

Larger sample budgets benefit from higher sampling temperatures in LLMs, but what temperature tuning optimizes and why it works remain poorly understood. We seek to answer these questions: we pose decoding as pass@$k$ maximization subject to two constraints that encode critical decoding failure modes: an entropy floor preventing diversity collapse, and a cross-entropy ceiling preventing implausibility. We prove that this maximization takes the form of a single closed-form conditional sampling rule, the \emph{tilted temperature} $q^\star \propto \bigl(p e^{\eta V}\bigr)^{1/T}$. Here, the tilt comes from a verifier potential $V$ that quantifies how likely a partial generation is to eventually pass. Ordinary temperature sampling, verifier-greedy decoding, and reward-tilted policies represent special cases. We further show that, under a natural rule for scaling the diversity budget with sample size $k$, the resulting optimal temperature increases with $k$, turning empirical choice into a theorem. The optimum still needs the unknown verifier potential, which we estimate using two design approaches. In the online setting, our J-EOS algorithm jointly tracks the two constraint multipliers and learns the verifier potential from binary pass/ fail feedback alone. In the offline setting, we show that when the model is calibrated, its log-probability tracks correctness up to an affine map. Under this condition, the tilt collapses into the exponent and the optimum reduces to ordinary temperature sampling. Calibrated Temperature Decoding (CTD) then fits one scalar offline and samples with zero additional inference-time overhead relative to temperature sampling. Building on these decision rules, we design a practical decoding algorithm for code generation and evaluate it alongside CTD on benchmarks including HumanEval and MBPP, showing improvements over standard and adaptive decoding baselines.

==> adaptive2.tex <==

\section{Adaptive Optimization: Piecewise-in-Horizon Budgets}
\label{app:adaptive}

Program (PE) uses one diversity floor $\beta$ and one plausibility ceiling
$\gamma$ over the full horizon. To model position-adaptive decoding, we let
these budgets take a small number $D$ of values along the horizon. The main
structural fact is that the optimum remains in the tilted-temperature family:
each block receives its own pair $(T_d,\eta_d)$. The global result of
Theorem~\ref{thm:tilt} is recovered at $D=1$.

This extension is useful for interpreting practical adaptive decoders. A
position-dependent temperature schedule can exploit coarse variation across
the horizon, while a value-aware tilted decoder can additionally react to the
state of the current prefix. The block model isolates the first effect.

\subsection{Block program and optimum}

Fix cut points
\[
0=t_0<t_1<\cdots<t_D=n,
\qquad
B_d:=\{t_{d-1}+1,\ldots,t_d\},
\qquad
n_d:=|B_d|.
\]
Each block carries its own diversity and plausibility budgets
$(\beta_d,\gamma_d)$. The block-constrained problem is
\begin{equation}
\label{eq:PED}
\max_q\ u_q
\quad\text{s.t.}\quad
\frac{1}{n_d}\sum_{t\in B_d}
\E_{w^{t-1}\sim q}
H\!\bigl(q_t(\cdot\mid w^{t-1})\bigr)\ge \beta_d,
\end{equation}
and
\begin{equation}
-\frac{1}{n_d}\sum_{t\in B_d}
\E_{w^{t-1}\sim q}
\Bigl[\sum_w q_t(w\mid w^{t-1})\log p_t(w\mid w^{t-1})\Bigr]
\le \gamma_d,
\qquad d=1,\ldots,D.
\tag{PE-$D$}
\end{equation}
As in (PE), maximizing $\passk$ is equivalent to maximizing the one-sample
success $u_q$ for fixed budgets.

Let $\mu_d>0$ and $\lambda_{0,d}>0$ denote the active block multipliers and
define
\[
\lambda_d:=\frac{\lambda_{0,d}}{n_d},
\qquad
\lambda_d^\star:=\frac{n_d\lambda_d}{\mu_d},
\qquad
\mu_d^\star:=\frac{n_d}{\mu_d},
\qquad
T_d:=\frac{1}{\lambda_d^\star},
\qquad
\eta_d:=\frac{\mu_d^\star}{\lambda_d^\star}.
\]
Write $d(t)$ for the block containing step $t$, set
$J_{n+1}(w^n):=U(w^n)$, and define the backward recursion
\begin{equation}
\label{eq:Jrec}
J_t(w^{t-1})
=
\frac{1}{\mu^\star_{d(t)}}
\log
\sum_{w\in W}
p_t(w\mid w^{t-1})^{\lambda^\star_{d(t)}}
\exp\!\Bigl(
\mu^\star_{d(t)}J_{t+1}(w^{t-1}w)
\Bigr).
\end{equation}
Let
\[
V_t(w\mid w^{t-1}):=J_{t+1}(w^{t-1}w).
\]

\begin{theorem}[$D$-block tilted temperature]
\label{thm:dblock}
Assume the block budgets are jointly attainable and all block entropy floors
are active. Then the optimum of \textup{(PE-$D$)} is
\begin{equation}
\label{eq:dblock-opt}
q_t^\star(w\mid w^{t-1})
\propto
p_t(w\mid w^{t-1})^{\lambda^\star_{d(t)}}
\exp\!\Bigl(
\mu^\star_{d(t)}V_t(w\mid w^{t-1})
\Bigr),
\end{equation}
or equivalently
\[
q_t^\star(w\mid w^{t-1})
\propto
\Bigl(
p_t(w\mid w^{t-1})
e^{\eta_{d(t)}V_t(w\mid w^{t-1})}
\Bigr)^{1/T_{d(t)}}.
\]
Thus the optimum remains tilted-temperature, with a pair
$(T_d,\eta_d)$ for each horizon block.
\end{theorem}

\begin{proof}[Proof sketch]
The proof is the proof of Theorem~\ref{thm:tilt} with position-dependent
dual prices. The Lagrangian still decomposes as a finite-horizon control
problem; only the entropy and log-likelihood coefficients are now piecewise
constant in $t$. Applying the Gibbs variational principle at each node gives
\eqref{eq:Jrec} and \eqref{eq:dblock-opt}. Strong duality and complementary
slackness then identify the block prices with the active budgets.
\end{proof}

\subsection{What changes at block boundaries}

For $D=1$, the backward recursion can be flattened into the single
sequence-level free energy used in the main text. With different block prices,
that flattening generally fails across a block boundary: the continuation
computed in one block is re-tempered by the prices of the preceding block.

For example, with two blocks and a boundary at $t_1$, for $t\in B_1$,
\begin{equation}
\label{eq:nested-D2}
V_t
=
\frac{1}{\mu_1^\star}
\log
\sum_{w_{t+1:t_1}}
\prod_{s=t+1}^{t_1}p_s^{\lambda_1^\star}
\left(
\sum_{w_{t_1+1:n}}
\prod_{s=t_1+1}^{n}p_s^{\lambda_2^\star}
e^{\mu_2^\star U(w^n)}
\right)^{\mu_1^\star/\mu_2^\star}.
\end{equation}
The inner and outer log-sum-exp operators merge only when the corresponding
diversity prices agree. Thus the Bellman recursion remains simple, but the
sequence law acquires seam corrections.

\begin{proposition}[Sequence-level block correction]
\label{prop:seq-dblock}
Under Theorem~\ref{thm:dblock},
\begin{equation}
\label{eq:seq-dblock}
q^\star(w^n)
\propto
\left(
\prod_{d=1}^{D}
\prod_{t\in B_d}
p_t(w_t\mid w^{t-1})^{\lambda_d^\star}
\right)
\exp\!\left(
\mu_D^\star U(w^n)
+
\sum_{d=1}^{D-1}
(\mu_d^\star-\mu_{d+1}^\star)
J_{t_d+1}(w^{t_d})
\right).
\end{equation}
When all $\mu_d^\star$ coincide, the seam corrections vanish. If, in
addition, all $\lambda_d^\star$ coincide, \eqref{eq:seq-dblock} reduces to
the sequence-level law of Corollary~1.
\end{proposition}

\begin{proof}
Multiplying the conditionals in \eqref{eq:dblock-opt} yields
\[
q^\star(w^n)
=
\left(\prod_t p_t^{\lambda^\star_{d(t)}}\right)
\exp\!\left(
\sum_{t=1}^n
\mu^\star_{d(t)}(J_{t+1}-J_t)
\right).
\]
The sum telescopes within each block. Collecting the remaining boundary terms
gives \eqref{eq:seq-dblock}.
\end{proof}

\subsection{Connection to sample budget and practical adaptive decoding}

For a fixed block schedule
$\{(\beta_d,\gamma_d)\}_{d=1}^D$, the optimizer remains independent of $k$,
because $\passk(q)=1-(1-u_q)^k$ is monotone in $u_q$. As in the global case,
$k$ affects the decoder only through how the diversity budgets are selected.
Hence the ``larger $k$ wants hotter'' mechanism can be applied blockwise:
larger sample budgets may justify more diversity, while the block structure
determines where that diversity is spent.

The distinction between block adaptation and value-aware adaptation is also
useful experimentally. A block temperature schedule can react to position but
not to the realized prefix within a block. By contrast, the continuation
potential $V_t(w\mid w^{t-1})$ is state dependent. This gives a direct
interpretation of the practical comparisons in Section~4: AdapT represents
position-dependent temperature adaptation, while TMAD-Gated uses similar
intervention opportunities but additionally incorporates confidence and a
continuation-success proxy. The block model therefore isolates the benefit
available from coarse position-dependent temperature schedules; any remaining
advantage from explicit continuation information corresponds to structure that
a fixed block schedule cannot express.

Under perfect calibration, a block-temperature decoder remains especially
simple when the diversity price is shared across blocks: the verifier
contribution folds into the block exponents, while unequal diversity prices
produce the seam terms in \eqref{eq:seq-dblock}. More generally, those seam
corrections require explicit continuation-value information rather than a
temperature schedule alone.


==> callibration2.tex <==
\section{Proof of Theorems~\ref{thm:collapse} and \ref{thm:partial}}\label{app:partial}
Throughout we use the \emph{sequence-level} calibration of Definition~\ref{def:calib},
\begin{equation}\label{eq:calib-recall}
U(w^n)=s\,\bar\ell(w^n)+\bar c+\bar r(w^n),\qquad
\bar\ell(w^n)=\tfrac1n\log p(w^n),\qquad \sup_{w^n}|\bar r(w^n)|\le\varepsilon,
\end{equation}
and write $\CE(q):=-\tfrac1n\E_q[\log p(w^n)]$, $\bar H(q):=\tfrac1n\sum_t\E_{w^{t-1}\sim q}\,H\bigl(q_t(\cdot\mid w^{t-1})\bigr)$. Every distribution on $\W^n$ factorizes autoregressively, so~\eqref{eq:PE} is an optimization over $\Delta(\W^n)$; we use this freely. Since $p_t\ge\rho>0$, $p(w^n)\ge\rho^n>0$ on all of $\W^n$.

\begin{lemma}[Sequence-level form of the budgets]\label{lem:app-seqbudgets}
For every policy $q$:
\textup{(a)} $-\tfrac1n\sum_t\E_{w^{t-1}\sim q}\bigl[\sum_w q_t\log p_t\bigr]=\CE(q)$;
\textup{(b)} $\bar H(q)=\tfrac1n H(q)$;
\textup{(c)} under~\eqref{eq:calib-recall}, $u_q=\bar c-s\,\CE(q)+\E_q[\bar r]$.
\end{lemma}
\begin{proof}
(a) $\E_q[\log p(w^n)]=\sum_t\E_q[\log p_t(w_t\mid w^{t-1})]=\sum_t\E_{w^{t-1}\sim q}\bigl[\sum_w q_t(w\mid w^{t-1})\log p_t(w\mid w^{t-1})\bigr]$ by the tower property. (b) Chain rule of entropy. (c) Take $\E_q$ in~\eqref{eq:calib-recall} and use $\E_q[s\bar\ell]=\tfrac sn\E_q\log p=-s\,\CE(q)$.
\end{proof}

\begin{lemma}[Tempered family]\label{lem:app-tempered}
For $a\ge0$ let $q_a(w^n)\propto p(w^n)^a$ and $A(a):=\log\sum_{w^n}p(w^n)^a$. Then:
\begin{enumerate}[label=\textup{(\roman*)},leftmargin=2.2em]
\item $H(q_a)=A(a)-aA'(a)$ and $\tfrac{d}{da}H(q_a)=-a\,\Var_{q_a}(\log p)$.
\item If $p(w^n)$ has a unique mode, then $H(q_0)=n\log|\W|$, $H(q_a)\to0$ as $a\to\infty$, and $a\mapsto H(q_a)$ is continuous and strictly decreasing on $(0,\infty)$. Hence for every $\beta\in(0,\log|\W|)$ there is a unique $a_\beta>0$ with $\bar H(q_{a_\beta})=\beta$, and $\beta\mapsto a_\beta$ is continuous and strictly decreasing.
\item \textup{(Entropy-constrained CE minimality.)} For every $q\in\Delta(\W^n)$ with $\bar H(q)\ge\beta$, $\CE(q)\ge\CE(q_{a_\beta})$, with equality iff $q=q_{a_\beta}$.
\end{enumerate}
\end{lemma}
\begin{proof}
(i) $\log q_a=a\log p-A(a)$ and $A'(a)=\E_{q_a}[\log p]$, so $H(q_a)=-\E_{q_a}[a\log p-A(a)]=A-aA'$; differentiating, $\tfrac{d}{da}H(q_a)=-aA''(a)=-a\Var_{q_a}(\log p)$.
(ii) $q_0$ is uniform on $\W^n$ and $q_a$ concentrates on the unique mode as $a\to\infty$. A unique mode with $|\W^n|\ge2$ makes $\log p$ non-constant, and $q_a$ has full support, so $\Var_{q_a}(\log p)>0$ and (i) gives strict decrease. The claims on $a_\beta$ follow from continuity and strict monotonicity, using (b) of Lemma~\ref{lem:app-seqbudgets}.
(iii) For any $q$, $0\le\mathrm{KL}(q\,\|\,q_{a_\beta})=-H(q)-a_\beta\E_q[\log p]+A(a_\beta)$. Hence, using $H(q)\ge n\beta=H(q_{a_\beta})$ and (i),
\[
a_\beta\,n\,\CE(q)=-a_\beta\E_q[\log p]\ \ge\ H(q)-A(a_\beta)\ \ge\ H(q_{a_\beta})-A(a_\beta)=-a_\beta\E_{q_{a_\beta}}[\log p]=a_\beta\,n\,\CE(q_{a_\beta}).
\]
Divide by $a_\beta n>0$. Equality forces $\mathrm{KL}(q\|q_{a_\beta})=0$.
\end{proof}
Part (iii) uses no calibration: it is the maximum-entropy characterization of tempering, read as a cross-entropy minimization.

\begin{proof}[Proof of Theorem~\ref{thm:collapse}]
With $\varepsilon=0$, Lemma~\ref{lem:app-seqbudgets}(c) gives $u_q=\bar c-s\,\CE(q)$. Since $\passk(q)=1-(1-u_q)^k$ is strictly increasing in $u_q$ and $s>0$, for every $k$ program~\eqref{eq:PE} is equivalent to minimizing $\CE(q)$ over $\mathcal F:=\{q:\bar H(q)\ge\beta,\ \CE(q)\le\gamma\}$. By Lemma~\ref{lem:app-tempered}(iii), $\inf\{\CE(q):\bar H(q)\ge\beta\}=\CE(q_{a_\beta})$, attained only at $q_{a_\beta}$. If $\gamma<\CE(q_{a_\beta})$, then $\mathcal F=\emptyset$. If $\gamma\ge\CE(q_{a_\beta})$, then $q_{a_\beta}\in\mathcal F\subseteq\{\bar H\ge\beta\}$, so it is the unique minimizer over $\mathcal F$. This proves feasibility iff $\gamma\ge\CE(q_{a_\beta})$; $\gamma$ enters only through feasibility.

\emph{Relation to Theorem~\ref{thm:tilt}.} With $\lambda^\star=0$ and $\mu^\star=na_\beta/s$, the sequence law of Corollary~\ref{cor:seqtilt} in $(\lambda^\star,\mu^\star)$ form is $p^{\lambda^\star}e^{\mu^\star U}\propto e^{\mu^\star\frac sn\log p}=p^{a_\beta}$. This is the boundary case of Theorem~\ref{thm:tilt} in which the ceiling is slack (its multiplier vanishes) and the entropy multiplier is $\mu_E=n/\mu^\star=s/a_\beta>0$. The $(T,\eta)$ parametrization degenerates there, and the exponent is carried by $\mu^\star$ alone.

\emph{Conditionals.} Write $p(w^n)=p(w^t)\prod_{s>t}p_s(w_s\mid w^{s-1})$ and marginalize the future:
\begin{equation}\label{eq:pertoken-app}
q^\star_t(w\mid w^{t-1})=\frac{\sum_{w_{t+1:n}}p(w^n)^{a_\beta}}{\sum_{w,w_{t+1:n}}p(w^n)^{a_\beta}}\ \propto\ p_t(w\mid w^{t-1})^{a_\beta}\,\Psi^{(a_\beta)}_t(w^{t-1}w),
\end{equation}
the prefix factor $p(w^{t-1})^{a_\beta}$ cancelling, with $\Psi^{(a)}_t$ as in~\eqref{eq:pertoken} and $\Psi^{(a)}_n\equiv1$. Under prefix-independent conditionals, $\Psi^{(a)}_t=\prod_{s>t}\sum_{w_s}p_s(w_s)^a$ does not depend on the prefix or on $w$, leaves the normalizer, and~\eqref{eq:pertoken-app} reduces to~\eqref{eq:tempopt}.

At $s=0$, $u_q\equiv\bar c$ and every feasible $q$ is optimal. Finally, $\beta\mapsto a_\beta$ is strictly decreasing by Lemma~\ref{lem:app-tempered}(ii), which is the monotonicity used after Theorem~\ref{thm:collapse}.
\end{proof}

\begin{remark}[Why sequence-level scoring]\label{rem:app-tokenvsseq}
Lemma~\ref{lem:app-seqbudgets}(c) is exact because the calibration score $\bar\ell$ is the same functional as the plausibility ceiling, by Lemma~\ref{lem:app-seqbudgets}(a). A token-level hypothesis $V_t(w)=s\log p_t(w)+c_t$ does not yield it. Under~\eqref{eq:calib-recall} with $\varepsilon=0$, the potential of Lemma~1 at the prices above is
$V_t(w\mid w^{t-1})=\bar c+\tfrac sn\log p(w^{t-1})+\tfrac sn\log p_t(w\mid w^{t-1})+\tfrac1{\mu^\star}\log\Psi^{(a_\beta)}_t(w^{t-1}w)$:
affine in $\log p_t$ with slope $s/n$, plus the remaining-horizon term. Sequence-level scoring is also exactly what~\eqref{eq:ols} estimates.
\end{remark}
\begin{lemma}[Sharp mean-difference inequality]\label{lem:meandiff}
For probability measures $P,Q$ on a common space and any bounded $g$,
$\bigl|\E_P[g]-\E_Q[g]\bigr|\le\bigl(\sup g-\inf g\bigr)\,\TV(P,Q)$.
\end{lemma}
\begin{proof}
For any constant $c$, $\E_P[g]-\E_Q[g]=\sum_x(P-Q)(x)(g(x)-c)$. Take $c=\tfrac12(\sup g+\inf g)$, so $|g-c|\le\tfrac12(\sup g-\inf g)$, and use $\sum_x|P(x)-Q(x)|=2\TV(P,Q)$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:partial}]
Let $\tilde q:=q_{a_\beta}$, which is defined for $s\ge0$ since it depends only on $(p,\beta)$.

\textbf{(i)} By Lemma~\ref{lem:app-tempered}(ii), $\bar H(\tilde q)=\beta$, and $\CE(\tilde q)\le\gamma$ by hypothesis, so $\tilde q$ is feasible and $u_{q^\star}\ge u_{\tilde q}$. The optimum $q^\star$ is feasible, so $\bar H(q^\star)\ge\beta$, and Lemma~\ref{lem:app-tempered}(iii) gives $\CE(q^\star)\ge\CE(\tilde q)$. By Lemma~\ref{lem:app-seqbudgets}(c) and $s\ge0$,
\[
u_{q^\star}-u_{\tilde q}=s\bigl[\CE(\tilde q)-\CE(q^\star)\bigr]+\E_{q^\star}[\bar r]-\E_{\tilde q}[\bar r]\ \le\ \E_{q^\star}[\bar r]-\E_{\tilde q}[\bar r]\ \le\ 2\varepsilon.
\]
Lemma~\ref{lem:meandiff} sharpens the last step to $2\varepsilon\,\TV(q^\star,\tilde q)$.

\textbf{(ii)} The map $u\mapsto1-(1-u)^k$ has derivative $k(1-u)^{k-1}$, positive and non-increasing in $u$. By the mean value theorem there is $\xi\in[u_{\tilde q},u_{q^\star}]$ with $\passk(q^\star)-\passk(\tilde q)=k(1-\xi)^{k-1}(u_{q^\star}-u_{\tilde q})$. Since $\xi\ge u_{\tilde q}\ge u_{q^\star}-2\varepsilon$ by (i), $k(1-\xi)^{k-1}\le\sigma_k^{+}$. Combined with (i), the gap lies in $[0,2\varepsilon\sigma_k^{+}]$.

\textbf{(iii)} For $v\in(0,1)$ let $\sigma_v(k):=k(1-v)^{k-1}$, $k>0$. Then $\tfrac{d}{dk}\log\sigma_v(k)=\tfrac1k+\log(1-v)$, which is positive for $k<k_v:=-1/\log(1-v)$ and negative after. So $\sigma_v$ is strictly unimodal with maximizer $k_v$, and $\sigma_v(k)\to0$ as $k\to0^+$ and as $k\to\infty$. With $v=u_{q^\star}-2\varepsilon\in(0,1)$ we get $\sigma^{+}_k=\sigma_v(k)$, peaking at $k_v=1/v+O(1)$. Hence for every $\delta>0$ the set $\{k:2\varepsilon\sigma_k^{+}>\delta\}$ is a bounded (possibly empty) interval, and outside it $\tilde q$ is $\delta$-optimal by (ii).
\end{proof}


==> ctd2.tex <==
\section{Proof of Theorem~\ref{thm:ctd}: suboptimality and certification of CTD}\label{app:ctd}
We keep the notation of Appendix~\ref{app:partial}. The deployed policy is $\hat q_{\mathrm{CTD}}=q^{\mathrm{temp}}_{\hat a}$, per-token temperature at the Phase-2 exponent. The regression of Phase~1 does \emph{not} enter the policy: $\hat a$ depends only on $(p,\beta)$. The proof therefore has a deterministic part, the $\passk$ bound, and a stochastic part, the probability that Phase~1 certifies.

\paragraph{Part A: the deterministic bound.}
The proof uses only the following property of Phase~2:
\begin{equation}\label{eq:app-floor}
\bar H(\hat q_{\mathrm{CTD}})\ \ge\ \beta,\qquad \CE(\hat q_{\mathrm{CTD}})\le\gamma,
\end{equation}
which holds with equality in the entropy when $\hat a$ is the exact root. Then:
\begin{enumerate}[label=\textup{(\alph*)},leftmargin=2.2em]
\item $\hat q_{\mathrm{CTD}}$ is feasible, so $u_{q^\star}\ge u_{\hat q_{\mathrm{CTD}}}$.
\item By Lemma~\ref{lem:app-tempered}(iii) applied to $\hat q_{\mathrm{CTD}}$, $\Delta_{\CE}=\CE(\hat q_{\mathrm{CTD}})-\CE(q_{a_\beta})\ge0$, with equality iff $\hat q_{\mathrm{CTD}}=q_{a_\beta}$.
\item Applied to $q^\star$, which is feasible, the same lemma gives $\CE(q^\star)\ge\CE(q_{a_\beta})$.
\end{enumerate}
By Lemma~\ref{lem:app-seqbudgets}(c) and $s\ge0$,
\[
u_{q^\star}-u_{\hat q_{\mathrm{CTD}}}
= s\bigl[\CE(\hat q_{\mathrm{CTD}})-\CE(q^\star)\bigr]+\E_{q^\star}[\bar r]-\E_{\hat q_{\mathrm{CTD}}}[\bar r]
\ \le\ s\bigl[\CE(\hat q_{\mathrm{CTD}})-\CE(q_{a_\beta})\bigr]+2\varepsilon
= s\Delta_{\CE}+2\varepsilon .
\]
As in Theorem~\ref{thm:partial}(ii), the mean value theorem with $\xi\ge u_{q^\star}-(s\Delta_{\CE}+2\varepsilon)$ gives
$0\le\passk(q^\star)-\passk(\hat q_{\mathrm{CTD}})\le\sigma_k^{++}(s\Delta_{\CE}+2\varepsilon)$, which is~\eqref{eq:ctdbound}.

\emph{When $\Delta_{\CE}=0$.} Under prefix-independent conditionals, $\Psi^{(a)}_t$ is token-free for every $a$, so by~\eqref{eq:pertoken-app} $q^{\mathrm{temp}}_a=q_a$ for all $a$. Then $\bar H(\hat q_{\mathrm{CTD}})=\beta$ forces $\hat a=a_\beta$ by Lemma~\ref{lem:app-tempered}(ii), and $\Delta_{\CE}=0$. In general, $\Delta_{\CE}$ is the cross-entropy price, at fixed entropy, of dropping the remaining-horizon factor $\Psi^{(a)}_t$.

\begin{remark}[Monte-Carlo root in Phase~2]
Part~A needs only~\eqref{eq:app-floor}, not an exact root. If Phase~2 estimates $\bar H(q^{\mathrm{temp}}_a)$ to accuracy $\tau$ and bisects on the conservative target $\beta+\tau$, then~\eqref{eq:app-floor} holds on the accuracy event, and the extra slack enters the bound only through a larger $\Delta_{\CE}$.
\end{remark}

\paragraph{Part B: certification probability.}
Write $s_{\mathrm{spr}}^2=\Var(\bar\ell)\ge s_0^2$ and $s_{\mathrm{pop}}:=\Cov(\bar\ell,U)/\Var(\bar\ell)$.

\emph{Population slope} (Proposition~\ref{prop:ident}). By~\eqref{eq:calib-recall}, $\Cov(\bar\ell,U)=s\Var(\bar\ell)+\Cov(\bar\ell,\bar r)$. Since $|\bar r|\le\varepsilon$, Cauchy--Schwarz gives $|\Cov(\bar\ell,\bar r)|\le s_{\mathrm{spr}}\varepsilon$. Hence
\begin{equation}\label{eq:app-spop}
|s_{\mathrm{pop}}-s|\le\varepsilon/s_0=:C_0\varepsilon,\qquad |s_{\mathrm{pop}}|\le\tfrac{\sqrt{\Var U}}{s_{\mathrm{spr}}}\le\tfrac{1}{2s_0}.
\end{equation}

\emph{Concentration.} The empirical slope~\eqref{eq:ols} is $\hat s=\widehat\Cov/\widehat\Var$, a function of four empirical means: those of $\bar\ell\in[-B,0]$, $U\in\{0,1\}$, $\bar\ell U\in[-B,0]$, and $\bar\ell^2\in[0,B^2]$. By Hoeffding's inequality and a union bound, with probability at least $1-\delta/2$,
\[
|\widehat\Cov-\Cov|\vee|\widehat\Var-\Var|\le\eta_M:=c_1\bar B^2\sqrt{\tfrac{\log(8/\delta)}{N}},\qquad \bar B:=\max\{1,B\},
\]
with $c_1$ absolute. On this event, if $\eta_M\le s_0^2/2$, then $\widehat\Var\ge s_0^2/2$, and
\[
|\hat s-s_{\mathrm{pop}}|=\Bigl|\tfrac{\widehat\Cov-\Cov}{\widehat\Var}+s_{\mathrm{pop}}\tfrac{\Var-\widehat\Var}{\widehat\Var}\Bigr|
\le\frac{2\eta_M(1+|s_{\mathrm{pop}}|)}{s_0^2}\le\frac{C_s}{2}\sqrt{\tfrac{\log(8/\delta)}{N}},
\qquad C_s:=\frac{4c_1\bar B^2}{s_0^2}\Bigl(1+\frac1{2s_0}\Bigr).
\]

\emph{Sign.} Suppose $s>C_0\varepsilon$ and choose $\delta:=8\exp\bigl(-N(s-C_0\varepsilon)^2/C_s^2\bigr)$, so that $\tfrac{C_s}{2}\sqrt{\log(8/\delta)/N}=\tfrac12(s-C_0\varepsilon)$.
The side condition holds automatically: by~\eqref{eq:app-spop},
\[
\eta_M=c_1\bar B^2(s-C_0\varepsilon)/C_s\le c_1\bar B^2|s_{\mathrm{pop}}|/C_s<s_0^2/8.
\]
On the event, $\hat s\ge s_{\mathrm{pop}}-\tfrac12(s-C_0\varepsilon)\ge\tfrac12(s-C_0\varepsilon)>0$, using $s_{\mathrm{pop}}\ge s-C_0\varepsilon$. Hence
\[
\Pr(\hat s\le0)\ \le\ \delta/2\ \le\ 8\exp\!\bigl(-N(s-C_0\varepsilon)^2/C_s^2\bigr),
\]
with $C_0=1/s_0$ and $C_s$ depending only on $(B,s_0)$. This is the second claim of Theorem~\ref{thm:ctd}. \hfill$\blacksquare$

\begin{remark}[What the estimate does and does not control]
Unlike an analysis in which $\hat s$ sets the exponent, the policy here does not depend on $\hat s$. As a result there is no $O(1/\sqrt{N})$ term in~\eqref{eq:ctdbound} and no horizon factor to cancel. The estimate $(\hat s,\hat\varepsilon)$ serves two purposes: it decides whether the calibrated regime applies, and $\hat\varepsilon$ provides an empirical residual diagnostic for the deployment gate.
\end{remark}


==> jeos.tex <==
\section{Proof of Theorems 2 and 3}
\label{app:thm23}

Throughout this appendix $\theta=(\lambda,\mu)^\top\in\Theta\subset\mathbb R^2$, $\ell_t(w):=\log p_t(w\mid w^{t-1})$,
$V_t(w):=V_t(w\mid w^{t-1})$, $\phi_t(w):=(\ell_t(w),V_t(w))^\top$, and
\[
q^\theta_t(w) \;=\; \frac{\exp\big(\lambda\,\ell_t(w)+\mu\,V_t(w)\big)}{\sum_{w'\in\mathcal W}\exp\big(\lambda\,\ell_t(w')+\mu\,V_t(w')\big)}
\;\propto\; p_t(w)^\lambda\,e^{\mu V_t(w)},
\]
as in Section~\ref{sec:tracking}, with cumulative constraint map
\[
F_t(\theta) \;=\;
\begin{pmatrix}
\sum_{i=1}^t \big(\mathrm{CE}(q^\theta_i,p_i)-\gamma\big)\\[2pt]
\sum_{i=1}^t \big(H(q^\theta_i)-\beta\big)
\end{pmatrix},
\]
so that the offline active KKT point $\theta^\star=(\lambda^\star,\mu^\star)$ satisfies $F_n(\theta^\star)=0$, the prefix
tracker satisfies $F_t(\theta_t)=0$ for every $t$, and $R_t:=F_t(\theta^\star)$, $R:=\max_{1\le t\le n}\|R_t\|_2$ as in the
main text. Throughout, $V_t$ is held fixed with respect to $\theta$, isolating the tracking question addressed here
from the separate question of how $V_t$ is estimated.

\subsection{Proof of Theorem~\ref{thm:prefix-tracking} (Prefix-price tracking)}

Recall Assumption~\ref{ass:jacobian}: for every $t$ at which \eqref{eq:prefix-root} is solved,
$J_t := \int_0^1 DF_t\big(\theta_t+s(\theta^\star-\theta_t)\big)\,ds$ satisfies $\sigma_{\min}(J_t)\ge ct$ for a constant
$c>0$ independent of $t$.

\begin{proof}
By the fundamental theorem of calculus along the segment joining $\theta_t$ and $\theta^\star$,
\[
F_t(\theta^\star) - F_t(\theta_t) \;=\; \int_0^1 DF_t\big(\theta_t+s(\theta^\star-\theta_t)\big)\,ds\;(\theta^\star-\theta_t)
\;=\; J_t\,(\theta^\star-\theta_t).
\]
Since $F_t(\theta_t)=0$ and $F_t(\theta^\star)=R_t$ by definition, this reads $R_t = J_t(\theta^\star-\theta_t)$. Taking
norms and using $\|J_t x\|_2 \ge \sigma_{\min}(J_t)\|x\|_2$,
\[
\|R_t\|_2 \;\ge\; \sigma_{\min}(J_t)\,\|\theta^\star-\theta_t\|_2 \;\ge\; ct\,\|\theta_t-\theta^\star\|_2,
\]
by Assumption~\ref{ass:jacobian}. Rearranging, and using $\|R_t\|_2\le R$ for every $t$, gives
$\|\theta_t-\theta^\star\|_2 \le \|R_t\|_2/(ct) \le R/(ct)$.
\end{proof}

\begin{remark}
No global uniqueness of the root of $F_t$ is assumed. The bound only requires that the particular root $\theta_t$
selected by the tracker and the offline point $\theta^\star$ are joined by a segment on which the averaged Jacobian
$J_t$ is uniformly nonsingular in the sense of Assumption~\ref{ass:jacobian}; this is exactly what the mean-value
step above uses.
\end{remark}

\subsection{A conditional KL perturbation lemma}

The bridge from the parameter-space guarantee of Theorem~\ref{thm:prefix-tracking} to a distributional and, ultimately,
a $\mathrm{pass@}k$ guarantee goes through the local geometry of the exponential family $q^\theta_t$, not through
summing total-variation distances directly (the KL-versus-TV discussion in Section~\ref{sec:tracking}). For $\theta\in\Theta$ let
$A_t(\theta) := \log\sum_{w\in\mathcal W}\exp\big(\theta^\top\phi_t(w)\big)$ be the log-partition function of $q^\theta_t$,
so that $\nabla A_t(\theta) = \mathbb E_{q^\theta_t}[\phi_t(W)]$ and $\nabla^2 A_t(\theta) = \mathrm{Cov}_{q^\theta_t}(\phi_t(W))$.

\begin{lemma}[Conditional KL perturbation]
\label{lem:kl-perturbation}
Under Assumption~\ref{ass:cov},
\[
D_{\mathrm{KL}}\big(q^{\theta_t}_t \,\big\|\, q^{\theta^\star}_t\big) \;\le\; \frac{M}{2}\,\|\theta_t-\theta^\star\|_2^2.
\]
\end{lemma}

\begin{proof}
For an exponential family with natural parameter $\theta$ and log-partition $A_t$, the KL divergence between two
members is exactly the Bregman divergence of $A_t$:
\[
D_{\mathrm{KL}}\big(q^{\theta_t}_t\,\|\,q^{\theta^\star}_t\big)
= A_t(\theta^\star) - A_t(\theta_t) - \nabla A_t(\theta_t)^\top(\theta^\star-\theta_t).
\]
By Taylor's theorem with integral remainder,
\[
A_t(\theta^\star) - A_t(\theta_t) - \nabla A_t(\theta_t)^\top(\theta^\star-\theta_t)
= \int_0^1 (1-s)\,(\theta^\star-\theta_t)^\top \nabla^2 A_t\big(\theta_t+s(\theta^\star-\theta_t)\big)(\theta^\star-\theta_t)\,ds.
\]
Since $\nabla^2 A_t(\theta) = \mathrm{Cov}_{q^\theta_t}(\phi_t(W))$, Assumption~\ref{ass:cov} bounds its largest
eigenvalue by $M$ at every point on the segment, so the integrand is at most
$(1-s)\,M\,\|\theta^\star-\theta_t\|_2^2$; integrating over $s\in[0,1]$ contributes a factor $\int_0^1(1-s)\,ds=\tfrac12$,
giving the claim.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:passk-tracking} (Sequence-law and pass@k stability)}

Let $Q$ denote the autoregressive sequence law induced by the online conditionals $\{q^{\theta_t}_t\}_{t=1}^n$, and
$Q^\star$ the sequence law induced by the offline optimum $\{q^{\theta^\star}_t\}_{t=1}^n$.

\begin{proof}
\emph{KL bound.} By the chain rule for relative entropy on autoregressive sequence laws,
\[
D_{\mathrm{KL}}(Q\,\|\,Q^\star) \;=\; \sum_{t=1}^n \mathbb E_Q\Big[D_{\mathrm{KL}}\big(q^{\theta_t}_t(\cdot\mid W^{t-1})\,\big\|\,q^{\theta^\star}_t(\cdot\mid W^{t-1})\big)\Big].
\]
Applying Lemma~\ref{lem:kl-perturbation} termwise, then Theorem~\ref{thm:prefix-tracking} ($\|\theta_t-\theta^\star\|_2\le R/(ct)$),
\[
D_{\mathrm{KL}}(Q\,\|\,Q^\star) \;\le\; \frac{M}{2}\sum_{t=1}^n \|\theta_t-\theta^\star\|_2^2
\;\le\; \frac{M}{2}\sum_{t=1}^n \frac{R^2}{c^2t^2}
\;=\; \frac{MR^2}{2c^2}\sum_{t=1}^n\frac1{t^2}
\;\le\; \frac{M\pi^2}{12\,c^2}\,R^2,
\]
using $\sum_{t=1}^\infty 1/t^2=\pi^2/6$.

\emph{TV and success-probability bounds.} Pinsker's inequality, $\mathrm{TV}(Q,Q^\star)\le\sqrt{\tfrac12 D_{\mathrm{KL}}(Q\|Q^\star)}$,
gives $\mathrm{TV}(Q,Q^\star) \le \tfrac{\pi\sqrt M}{2\sqrt6\,c}\,R$. Since $U:\mathcal W^n\to[0,1]$ is bounded,
\[
|u_Q - u_{Q^\star}| \;=\; \big|\mathbb E_Q[U]-\mathbb E_{Q^\star}[U]\big| \;\le\; \mathrm{TV}(Q,Q^\star) \;\le\; \frac{\pi\sqrt M}{2\sqrt6\,c}\,R.
\]

\emph{$\mathrm{pass@}k$ bounds.} With $g_k(u):=1-(1-u)^k$, $g_k'(u)=k(1-u)^{k-1}\in[0,k]$ for $u\in[0,1]$, so $g_k$ is
$k$-Lipschitz and $|\mathrm{pass@}k(Q)-\mathrm{pass@}k(Q^\star)| = |g_k(u_Q)-g_k(u_{Q^\star})| \le k\,|u_Q-u_{Q^\star}|$;
combined with $\mathrm{pass@}k\in[0,1]$ this gives the stated
$\big|\mathrm{pass@}k(Q)-\mathrm{pass@}k(Q^\star)\big| \le \min\big\{1,\ k\,\tfrac{\pi\sqrt M}{2\sqrt6\,c}R\big\}$.
For the sharper form, the mean value theorem gives $\xi$ between $u_Q$ and $u_{Q^\star}$ with
$|g_k(u_Q)-g_k(u_{Q^\star})| = k(1-\xi)^{k-1}|u_Q-u_{Q^\star}|$; since $k(1-u)^{k-1}$ is decreasing in $u$ and
$\xi\ge u_{\min}:=\min\{u_Q,u_{Q^\star}\}$, this is at most $k(1-u_{\min})^{k-1}|u_Q-u_{Q^\star}|$, giving
$\big|\mathrm{pass@}k(Q)-\mathrm{pass@}k(Q^\star)\big| \le k(1-u_{\min})^{k-1}\,\tfrac{\pi\sqrt M}{2\sqrt6\,c}\,R$.
\end{proof}

\begin{remark}[Reading $R$]
\label{rem:reading-R}
$R=\max_{t\le n}\|F_t(\theta^\star)\|_2$ measures the maximal prefix imbalance of the \emph{final, offline} prices: how
far $\theta^\star$ is from satisfying the length-$t$ truncated budgets, at the worst truncation point. Theorem~\ref{thm:passk-tracking}
is a deterministic stability statement -- small prefix residual implies small $\mathrm{pass@}k$ deviation -- rather than
a regret bound in the online-learning sense, since $V_t$ is held fixed throughout this appendix; Appendix~\ref{app:mc}
addresses the separate problem of estimating $V_t$ from terminal verifier feedback. Because $\mathrm{pass@}k\in[0,1]$,
any bound exceeding one is vacuous, which is why the loose form of the bound is explicitly truncated at $1$.
\end{remark}

==> lem1.tex <==

\section{Proof of Lemma 1 (Bellman Consistency)}
\label{app:lem1}

Recall from Section 2 that, for prices $\lambda^\star\ge0$ and $\mu^\star>0$, a step
$t\in\{1,\dots,n\}$, a prefix $w^{t-1}$ and a token $w$ (so $w_t=w$),
\begin{equation}\label{eq:B-Vdef}
  V_t(w\mid w^{t-1})\;=\;\frac{1}{\mu^\star}\log\!\!
  \sum_{w_{t+1:n}\in\W^{\,n-t}}\ \prod_{s=t+1}^{n}p_s(w_s\mid w^{s-1})^{\lambda^\star}\,
  e^{\mu^\star U(w^n)},\qquad w^n=(w^{t-1},w,w_{t+1:n}),
\end{equation}
with the convention that at $t=n$ the continuation set $\W^0$ is the single empty tuple
and the product is empty. It is convenient to name the partition sum inside the
logarithm: for a length-$t$ prefix $w^t$ $(1\le t\le n)$ set
\begin{equation}\label{eq:B-Phi}
  \Phi(w^t)\;:=\;\sum_{w_{t+1:n}\in\W^{\,n-t}}\ \prod_{s=t+1}^{n}
  p_s(w_s\mid w^{s-1})^{\lambda^\star}\, e^{\mu^\star U(w^n)},
  \qquad \Phi(w^n):=e^{\mu^\star U(w^n)},
\end{equation}
so that \eqref{eq:B-Vdef} reads $\Phi(w^t)=\exp\!\big(\mu^\star V_t(w_t\mid w^{t-1})\big)$.

\medskip
\noindent\textbf{Lemma 1 (Bellman consistency, restated).}\ \emph{For any
$\lambda^\star\ge0$, $\mu^\star>0$, step $t\in\{1,\dots,n-1\}$, prefix $w^{t-1}$ and token
$w$,}
\[
  V_t(w\mid w^{t-1})=\frac{1}{\mu^\star}\log\sum_{w'\in\W}
  p_{t+1}(w'\mid w^{t-1}w)^{\lambda^\star}\exp\!\big(\mu^\star V_{t+1}(w'\mid w^{t-1}w)\big),
\]
\emph{with terminal condition $V_n(w\mid w^{n-1})=U(w^{n-1},w)$; equivalently
$V_t=\tfrac{T}{\eta}\log Z_{t+1}(w^{t-1}w)$ with}
\[
  Z_{t+1}(w^{t-1}w)=\sum_{w'\in\W}
  \Big(p_{t+1}(w'\mid w^{t-1}w)\,e^{\eta V_{t+1}(w'\mid w^{t-1}w)}\Big)^{1/T}.
\]
\emph{The recursion involves only $(p,U,\lambda^\star,\mu^\star)$, so $V$ exists, is
unique, and is obtained by one backward sweep over prefix states.}

\begin{proof}
\textbf{Well-posedness.} Fix $t$ and $w^t$. Since $\rho\le p_s(\cdot\mid w^{s-1})\le1$ and
$U\in[0,1]$, every summand of \eqref{eq:B-Phi} lies in
$\big[\rho^{\lambda^\star(n-t)},\,e^{\mu^\star}\big]$, and the index set $\W^{\,n-t}$ is
finite and nonempty. Hence
\begin{equation}\label{eq:B-bounds}
  0\;<\;\rho^{\lambda^\star(n-t)}\;\le\;\Phi(w^t)\;\le\;|\W|^{\,n-t}e^{\mu^\star}\;<\;\infty,
\end{equation}
so $V_t=(\mu^{\star})^{-1}\log\Phi(w^t)$ is finite for every $(t,w^{t-1},w)$, with
\[
  -\frac{\lambda^\star(n-t)}{\mu^\star}\log\frac1\rho\;\le\;V_t(w\mid w^{t-1})\;\le\;
  1+\frac{n-t}{\mu^\star}\log|\W| .
\]
(The two-sided bound \eqref{eq:B-bounds} is what makes the log-space form legitimate.)

\smallskip
\textbf{Recursion.} Fix $t\in\{1,\dots,n-1\}$ and a length-$t$ prefix $w^t=(w^{t-1},w)$.
Separate the first continuation token $w_{t+1}=w'$ and factor out
$p_{t+1}(w'\mid w^t)^{\lambda^\star}$, which is constant in $w_{t+2:n}$:
\begin{align*}
  \Phi(w^t)&=\sum_{w'\in\W}p_{t+1}(w'\mid w^t)^{\lambda^\star}
  \underbrace{\sum_{w_{t+2:n}}\ \prod_{s=t+2}^{n}p_s(w_s\mid w^{s-1})^{\lambda^\star}
  e^{\mu^\star U(w^n)}}_{=\ \Phi(w^t w')}\\
  &\;=\;\sum_{w'\in\W}p_{t+1}(w'\mid w^t)^{\lambda^\star}\,\Phi(w^tw'),
\end{align*}
where the brace equals $\Phi(w^tw')$ because for $s\ge t+2$ the factors
$p_s(w_s\mid w^{s-1})$ and the verifier $U(w^n)$ depend on $w_{t+1}$ only through the
now-fixed conditioning prefix $w^tw'$. Substituting
$\Phi(w^tw')=e^{\mu^\star V_{t+1}(w'\mid w^t)}$ and taking $\mu^{\star-1}\log$ yields the
stated recursion. At $t=n$ the empty-product convention gives
$\Phi(w^n)=e^{\mu^\star U(w^n)}$, hence $V_n(w\mid w^{n-1})=U(w^{n-1},w)$.

\smallskip
\textbf{Equivalent $(T,\eta)$ form.} With $\lambda^\star=1/T$ and $\mu^\star=\eta/T$
(so $\eta>0$ whenever $\mu^\star>0$),
\[
  p_{t+1}(w'\mid w^{t-1}w)^{\lambda^\star}e^{\mu^\star V_{t+1}(w'\mid w^{t-1}w)}
  =\Big(p_{t+1}(w'\mid w^{t-1}w)\,e^{\eta V_{t+1}(w'\mid w^{t-1}w)}\Big)^{1/T},
\]
so the sum in the recursion is exactly $Z_{t+1}(w^{t-1}w)$ --- the per-node normalizer of
the tilted-temperature step of Theorem 1 --- and $\mu^{\star-1}=T/\eta$ gives
$V_t=\tfrac{T}{\eta}\log Z_{t+1}(w^{t-1}w)$.

\smallskip
\textbf{Existence, uniqueness, backward sweep.} The closed form \eqref{eq:B-Vdef}
exhibits $V$ explicitly, so it exists. The recursion expresses $V_t$ through $V_{t+1}$
alone and the terminal condition fixes $V_n=U$; reading the layers
$t=n,n-1,\dots,1$ determines every $V_t$ exactly once. Any $V'$ obeying the recursion and
the terminal condition equals $V$ by downward induction on $t$ (they agree at $t=n$; if
they agree at $t+1$, the recursion forces agreement at $t$), giving uniqueness. As the
right-hand side involves only $(p,U,\lambda^\star,\mu^\star)$ and no policy $q$, $V$ is a
deterministic function of the instance and the two prices, computed by a single backward
pass of $n$ layers with no self-consistency condition to solve.
\end{proof}

\paragraph{$V_t$ is a free energy, not an ordinary conditional average.}
The potential $V_t$ is a log-partition quantity over tilted continuations rather than
an ordinary conditional expectation of the terminal verifier. This distinction is
important because the optimal decoder of Theorem 1 tilts directly on $V_t$. Four
facts summarize its structure.

\emph{(i) At the terminal step $V_t$ reduces to the verifier.}
When $t=n$ the continuation is empty and
\[
  V_n(w\mid w^{n-1})=U(w^{n-1},w).
\]

\emph{(ii) $V_t$ is a log-partition function.} Fix a committed pair
$w^t=(w^{t-1},w)$, let
$S_t(w^t):=\sum_{w_{t+1:n}}\prod_{s>t}p_s(w_s\mid w^{s-1})^{\lambda^\star}$
be the total tempered mass of its continuations, and let
$\nu_t(\cdot\mid w^t)$ be the probability measure on $\W^{n-t}$ proportional to
$\prod_{s>t}p_s(w_s\mid w^{s-1})^{\lambda^\star}$. Then \eqref{eq:V-def} reads
\begin{align}
\label{eq:V-logpart}
  V_t(w\mid w^{t-1})
  &\;=\;\frac{1}{\mu^\star}\log S_t(w^t)\;+\;\frac{1}{\mu^\star}\log
  \E_{\nu_t}\!\big[e^{\mu^\star U(w^n)}\big]\\
  &\;=\;\frac{1}{\mu^\star}\log S_t(w^t)+\E_{\nu_t}[U]
  +\frac{\mu^\star}{2}\Var_{\nu_t}(U)+O(\mu^{\star2}). 
  \nonumber
\end{align}
When $\lambda^\star=1$ (equivalently $T=1$), $\nu_t$ is the base-model
continuation law and $S_t\equiv1$, so as $\mu^\star\to0$,
\[
  V_t(w\mid w^{t-1})
  \longrightarrow
  \E_{w_{t+1:n}\sim p}\!\big[U(w^n)\mid w^t\big].
\]
At any other temperature $S_t$ need not equal one and the first term in
\eqref{eq:V-logpart} remains. This is harmless for the decoder: only the product
$\mu^\star V_t$ enters the optimum, and by \eqref{eq:V-logpart} it converges to
$\log S_t$ as $\mu^\star\downarrow0$.

\emph{(iii) $V_t$ is not a probability.} From \eqref{eq:V-def},
$p_s^{\lambda^\star}\le1$, $p_s\ge\rho$, and $U\in[0,1]$ give the explicit range
\[
  -\frac{\lambda^\star (n-t)}{\mu^\star}\,\log\frac1\rho
  \;\le\; V_t(w\mid w^{t-1})\;\le\;
  1+\frac{(n-t)}{\mu^\star}\,\log|\W| ,
\]
so $V_t$ need not lie in $[0,1]$.

\begin{remark}[Degenerate prices, and what $\eta=0$ actually gives]\label{rem:B-degenerate}
The lemma assumes $\mu^\star>0$, equivalently $\eta>0$. At $\mu^\star=0$ the definition
\eqref{eq:B-Vdef} is a $0/0$ and $V_t$ is undefined; what survives is the product
$\mu^\star V_t$, which is the only way $V_t$ enters the optimum. Taking the limit $\mu^\star\downarrow 0$ in
\eqref{eq:B-Phi} gives $\mu^\star V_t\to\log S_t(w^t)$, with
$S_t(w^t)=\sum_{w_{t+1:n}}\prod_{s>t}p_s(w_s\mid w^{s-1})^{\lambda^\star}$ the tempered
continuation mass of Section 2, so as $\mu^\star\downarrow0$ the tilted step of Theorem 1
becomes
\[
  q^\star_t(w\mid w^{t-1})\ \propto\ p_t(w\mid w^{t-1})^{1/T}\;S_t(w^{t-1}w).
\]
This is temperature sampling at the \emph{sequence} level --- telescoping (Corollary~\ref{cor:seqtilt})
gives $q^\star(w^n)\propto p(w^n)^{1/T}$ --- but it is \emph{not} per-token temperature
sampling: the extra factor $S_t(w^{t-1}w)$ steers toward branches whose continuation
carries cheap entropy, which is exactly the effect Corollary~\ref{cor:freeenergy} isolates. The two coincide
iff $S_t(w^{t-1}w)$ does not depend on $w$, i.e.\ at $n=1$, at $T=1$, or when the base
conditionals are prefix-independent (the i.i.d.-token regime of \cite{sima2026}). At $n\ge2$ with prefix-dependent conditionals
the factor is not constant.
\end{remark}


==> mc.tex <==
\section{Online Estimation of the Verifier Potential in J-EOS}
\label{app:mc}

J-EOS needs an estimate of the Bellman potential $V_t(w\mid w^{t-1})$ from
terminal pass/fail feedback.  After the causal price-tracking pass of round $r$,
it has a sequence of prices $\theta_{r,t}=(\lambda_{r,t},\mu_{r,t})$,
$t=1,\dots,n$.  We freeze the resulting J-EOS decoder and use it as an
importance-sampling behavior policy.  This appendix states the corresponding
rollout identity, the step-only estimator used by Algorithm~\ref{alg:jeos}, and
the approximation introduced by collapsing prefixes into a table indexed only
by $(t,w)$.

\paragraph{Target prices and frozen behavior.}
At the end of round $r$, let
\[
\vartheta_r=(\lambda_r,\mu_r):=\theta_{r,n}, \qquad \mu_r>0,
\]
be the price pair whose Bellman potential we want to estimate.  Freeze the
within-round prices $\{\theta_{r,t}\}_{t=1}^n$ and define the behavior policy
\begin{equation}
 b_{r,t}(w\mid w^{t-1})
 :=
 \frac{p_t(w\mid w^{t-1})^{\lambda_{r,t}}
       \exp\!\big(\mu_{r,t}\widehat V^{\rm prev}_t(w)\big)}
      {\sum_{a\in\W}p_t(a\mid w^{t-1})^{\lambda_{r,t}}
       \exp\!\big(\mu_{r,t}\widehat V^{\rm prev}_t(a)\big)} .
\label{eq:jeos-behavior}
\end{equation}
After freezing \eqref{eq:jeos-behavior}, draw a fresh batch of $m$ independent
rollouts from $b_r$.  Using a fresh batch is important: the causal trajectory
used to construct $\theta_{r,1:n}$ is adaptive and is not, in general, an i.i.d.
draw from the subsequently frozen behavior policy.

For a fixed target pair $\vartheta=(\lambda,\mu)$, define the Bellman partition
function after committing to $(w^{t-1},w)$ by
\begin{equation}
 Z^{\vartheta}_{t+1}(w^{t-1}w)
 :=
 \sum_{w_{t+1:n}}
 \left[\prod_{s=t+1}^n
 p_s(w_s\mid w^{s-1})^{\lambda}\right]
 e^{\mu U(w^n)},
 \qquad
 V_t^{\vartheta}(w\mid w^{t-1})
 =\frac1\mu\log Z^{\vartheta}_{t+1}(w^{t-1}w).
\label{eq:jeos-target-Z}
\end{equation}
This is exactly the potential of Lemma~\ref{lem:bellman}, evaluated at the
current target prices $\vartheta_r$.

\begin{proposition}[Off-policy rollout identity for J-EOS]
\label{prop:jeos-rollout}
Fix a round $r$ and target prices $\vartheta_r=(\lambda_r,\mu_r)$ with
$\mu_r>0$.  For every $t$, prefix $w^{t-1}$, and token $w$, if the behavior
policy has full support, then
\begin{equation}
Z^{\vartheta_r}_{t+1}(w^{t-1}w)
=
\E_{w_{t+1:n}\sim b_r}
\!\left[
 e^{\mu_r U(w^n)}
 \prod_{s=t+1}^{n}
 \frac{p_s(w_s\mid w^{s-1})^{\lambda_r}}
      {b_{r,s}(w_s\mid w^{s-1})}
 \ \middle|\ w^t
\right].
\label{eq:jeos-rollout}
\end{equation}
Consequently,
$V_t^{\vartheta_r}(w\mid w^{t-1})=\mu_r^{-1}\log
Z^{\vartheta_r}_{t+1}(w^{t-1}w)$.
\end{proposition}

\begin{proof}
Expand the expectation in \eqref{eq:jeos-rollout}.  The continuation probability
under $b_r$ is $\prod_{s>t}b_{r,s}(w_s\mid w^{s-1})$; it cancels the denominator
of the likelihood ratio, leaving
$\prod_{s>t}p_s(w_s\mid w^{s-1})^{\lambda_r}e^{\mu_rU(w^n)}$.
Summing over all continuations gives \eqref{eq:jeos-target-Z}.
\end{proof}

\paragraph{Step-only table used by J-EOS.}
Let $w^n_{(1)},\dots,w^n_{(m)}\stackrel{\rm iid}{\sim}b_r$ be the fresh rollout
batch and $U_{(j)}=U(w^n_{(j)})$.  For every visited cell $(t,w)$ define
\begin{align}
X^{(r,t)}_{(j)}
&:= e^{\mu_r U_{(j)}}
\prod_{s=t+1}^{n}
\frac{p_s(w_{(j),s}\mid w^{s-1}_{(j)})^{\lambda_r}}
     {b_{r,s}(w_{(j),s}\mid w^{s-1}_{(j)})},
\label{eq:jeos-weight}\\
\widehat Z^{(r)}_{t+1}(w)
&:=\frac{1}{N_{r,t}(w)}
\sum_{j:\,w_{(j),t}=w}X^{(r,t)}_{(j)},
\qquad
\widehat V^{(r)}_t(w)
:=\frac1{\mu_r}\log \widehat Z^{(r)}_{t+1}(w),
\label{eq:jeos-steponly}
\end{align}
where $N_{r,t}(w)=\#\{j:w_{(j),t}=w\}$.  Cells with
$N_{r,t}(w)=0$ retain their previous value (or are smoothed with a stated
pseudocount); they must not be assigned the logarithm of an empty sum.

Equation~\eqref{eq:jeos-steponly} is the update intended at the potential-update
line of Algorithm~\ref{alg:jeos}.  It requires storing the behavior probability
$b_{r,s}(w_{(j),s}\mid w^{s-1}_{(j)})$ for each sampled token, but it does not
require an oracle value of $(\lambda^\star,\mu^\star)$.

\paragraph{What the step-only table identifies.}
Because $\widehat V_t$ is indexed by $(t,w)$ rather than the full prefix, the
estimator cannot recover the exact prefix-conditioned potential in general.
Conditioning only on the event $w_t=w$ gives
\begin{equation}
\bar Z^{(r)}_{t+1}(w)
:=
\E_{w^{t-1}\sim b_r(\cdot\mid w_t=w)}
\!\left[Z^{\vartheta_r}_{t+1}(w^{t-1}w)\right]
=
\E_{w^{t-1}\sim b_r(\cdot\mid w_t=w)}
\!\left[e^{\mu_r V_t^{\vartheta_r}(w\mid w^{t-1})}\right],
\label{eq:jeos-marginal-target}
\end{equation}
and therefore
\begin{equation}
\bar V^{(r)}_t(w)
:=\frac1{\mu_r}\log \bar Z^{(r)}_{t+1}(w).
\label{eq:jeos-marginal-V}
\end{equation}
Thus the table converges to a behavior-weighted \emph{soft average} of the
prefix-conditioned potential.  This is an approximation intrinsic to the
$O(n|\W|)$ step-only representation, not a Monte-Carlo error.  It disappears
when $V_t^{\vartheta_r}(w\mid w^{t-1})$ is prefix-independent, and it can be
reduced by conditioning the value estimator on a richer state or learned hidden
representation.

\begin{theorem}[Per-round consistency of the J-EOS estimator]
\label{thm:jeos-consistency}
Fix a round $r$ and suppose that the $m$ rollouts are i.i.d.
from the frozen behavior policy $b_r$, that
$\Pr_{b_r}(W_t=w)\ge\rho_\star>0$ for all cells of interest, that
$p_s(a\mid h)\ge\rho>0$, and that
$b_{r,s}(a\mid h)\ge\kappa>0$ on the same support.  Set
\begin{equation}
\Delta_{r,t}
:=
 e^{\mu_r}\kappa^{-(n-t)}
 -\rho^{\lambda_r(n-t)}.
\label{eq:jeos-range}
\end{equation}
For $\delta\in(0,1)$, if
$m\ge\frac{8}{\rho_\star}\log\frac{2n|\W|}{\delta}$, then with probability
at least $1-\delta$, simultaneously for all visited cells,
\begin{equation}
\left|\widehat Z^{(r)}_{t+1}(w)-\bar Z^{(r)}_{t+1}(w)\right|
\le
\Delta_{r,t}
\sqrt{\frac{\log(4n|\W|/\delta)}{m\rho_\star}}.
\label{eq:jeos-concentration}
\end{equation}
Consequently $\widehat V^{(r)}_t(w)$ is consistent for
$\bar V^{(r)}_t(w)$.  Its logarithm produces the usual downward Jensen bias,
\begin{equation}
\E\!\left[\widehat V^{(r)}_t(w)\right]
=
\bar V^{(r)}_t(w)
-
\frac{\Var(\widehat Z^{(r)}_{t+1}(w))}
     {2\mu_r\,\bar Z^{(r)}_{t+1}(w)^2}
+o\!\left(\Var(\widehat Z^{(r)}_{t+1}(w))\right).
\label{eq:jeos-logbias}
\end{equation}
\end{theorem}

\begin{proof}
Conditional on $W_t=w$, the fresh rollouts are i.i.d. and the importance-weighted
quantity in \eqref{eq:jeos-weight} has mean
$\bar Z^{(r)}_{t+1}(w)$ by Proposition~\ref{prop:jeos-rollout} followed by the
prefix marginalization in \eqref{eq:jeos-marginal-target}.  Moreover,
$U\in[0,1]$ implies $e^{\mu_rU}\in[1,e^{\mu_r}]$, while
$p_s^{\lambda_r}/b_{r,s}\in[\rho^{\lambda_r},\kappa^{-1}]$.
Hence each weight lies in
$[\rho^{\lambda_r(n-t)},e^{\mu_r}\kappa^{-(n-t)}]$, an interval of width
$\Delta_{r,t}$.  A multiplicative Chernoff bound gives
$N_{r,t}(w)\ge\tfrac12m\rho_\star$ simultaneously with probability at least
$1-\delta/2$ under the stated sample-size condition.  Conditional on that
event, Hoeffding's inequality applied to each cell, followed by a union bound,
gives \eqref{eq:jeos-concentration}.  Finally,
$z\mapsto\mu_r^{-1}\log z$ is smooth on the positive range above; Jensen's
inequality gives the sign of the bias and a second-order Taylor expansion gives
\eqref{eq:jeos-logbias}.
\end{proof}

\begin{remark}[This does not by itself prove joint J-EOS convergence]
\label{rem:jeos-two-timescale}
Appendix~\ref{app:thm23} proves stability of the price tracker with the potential
held fixed.  The theorem above proves consistency of one potential update with
the target prices and behavior policy frozen within a round.  Combining these
two facts is a two-timescale tracking argument; it requires an additional
assumption controlling how quickly $\vartheta_r$ and the induced potential move
between rounds.  Therefore the present theory supports J-EOS as a per-round
price-tracking plus potential-estimation procedure, but it should not be stated
as a full no-regret or global-convergence theorem unless that extra argument is
added.
\end{remark}

\begin{remark}[Boundary case $\mu_r=0$]
The representation $V=\mu^{-1}\log Z$ is undefined at $\mu=0$.  Since J-EOS is
initialized at $\mu_0=0$, the first round should retain the zero-potential warm
start until the tracked solution enters the interior ($\mu_r>0$), or else the
implementation should separately track the log-partition product $\mu V$ near
the boundary.  The interior analysis in Section~\ref{sec:tracking} and
Appendix~\ref{app:thm23} already excludes the degenerate boundary case.
\end{remark}


==> prompt.tex <==
\providecommand{\X}{\mathcal{X}}
\providecommand{\Dist}{\mathcal{D}}
\providecommand{\Simp}{\Delta}
\providecommand{\W}{\mathcal{W}}
\providecommand{\E}{\mathbb{E}}
\providecommand{\Hbar}{\bar H}
\providecommand{\CE}{\mathrm{CE}}
\providecommand{\Vt}{\widetilde{V}}
\providecommand{\lamst}{\lambda^{\star}}
\providecommand{\must}{\mu^{\star}}
\providecommand{\qst}{q^{\star}}
\providecommand{\argmin}{\operatorname{arg\,min}}

\section{Prompt-Aware and Robust Formulations of (PE)}
\label{app:prompt}

\providecommand{\qst}{q^{\star}}
\providecommand{\argmin}{\operatorname{arg\,min}}


Program (PE) is written for a fixed prompt: $p_t(w\mid w^{t-1})$ already conditions on $x$,
so its optimum is a per-prompt object. In deployment a single decoder is applied across a
prompt distribution, and the natural objectives --- average and worst-case --- must be
written down explicitly. This appendix does that for three formulations and shows that each
is solved by the tilted-temperature family of Theorem~1 applied prompt-wise. The
formulations differ only in how the two prices $(T,\eta)$ are pinned: locally at each
prompt, globally across the prompt distribution, or globally at a least-favorable mixture.

Let $\X$ be the prompt space with reference distribution $\Dist$; take $\X$ finite (or
compact, with the usual continuity, so that the minima below are attained). For each
$x\in\X$ the model provides conditionals $p_t(\cdot\mid w^{t-1},x)\in\Simp(\W)$ with
$p_t\ge\rho>0$, and a possibly $x$-dependent verifier $U(\cdot,x):\W^n\to[0,1]$. A decoder
is a measurable map
\[
\Phi:\ (x,w^{t-1})\ \longmapsto\ q_t(\cdot\mid w^{t-1},x)\in\Simp(\W),\qquad t=1,\dots,n,
\]
i.e.\ it chooses a sampler at every prompt and prefix. Write the per-prompt quantities
\[
u_q(x):=\E_{w^n\sim q(\cdot\mid x)}\big[U(w^n,x)\big],
\qquad
\Hbar_q(x):=\frac1n\sum_t\E_{w^{t-1}\sim q}\,H\big(q_t(\cdot\mid w^{t-1},x)\big),
\]
\[
\CE_q(x):=-\frac1n\sum_t\E_{w^{t-1}\sim q}\Big[\textstyle\sum_w q_t\log p_t\Big].
\]
The observation that drives everything below: $u_q(x)$, $\Hbar_q(x)$ and $\CE_q(x)$ depend
on the decoder only through its restriction $q(\cdot\mid x)$ to prompt $x$. Distinct
prompts are coupled only if a constraint or the objective ties them together.

For prices $\lambda>0$, $\mu>0$ let $V^{\,x}_t(w\mid w^{t-1};\lambda,\mu)$ denote the
verifier potential of Lemma~1 built from the pair $\big(p(\cdot\mid x),U(\cdot,x)\big)$ at
those prices: it involves no policy, and is obtained by one backward sweep over prefix states
per prompt. We write $\varpi\in\Simp(\X)$ for a mixture over prompts, reserving $w$ for
tokens. We propose three prompt-level formulations:

\paragraph{(A) Average objective, per-prompt budgets.}
\begin{equation}\label{eq:A}
\max_{\Phi}\ \E_{x\sim\Dist}\big[u_q(x)\big]
\quad\text{s.t.}\quad
\Hbar_q(x)\ge\beta(x),\ \ \CE_q(x)\le\gamma(x)\ \ \text{for $\Dist$-a.e.\ }x.
\tag{A}
\end{equation}

\paragraph{(B) Average objective, pooled budgets.}
\begin{equation}\label{eq:B}
\max_{\Phi}\ \E_{x\sim\Dist}\big[u_q(x)\big]
\quad\text{s.t.}\quad
\E_{x\sim\Dist}\big[\Hbar_q(x)\big]\ge\beta,\ \
\E_{x\sim\Dist}\big[\CE_q(x)\big]\le\gamma.
\tag{B}
\end{equation}
One diversity budget and one plausibility budget are shared across the whole prompt
distribution --- the deployment regime, where a single temperature is spent over the
benchmark. This is the formulation the experiments of Section~4 instantiate: one
cross-entropy budget anchored at a reference temperature, one deployed $T$, applied across
all tasks.

\paragraph{(C) Worst-case prompt (robust / distributionally robust).}
\begin{equation}\label{eq:C}
\max_{\Phi}\ \min_{x\in\X}\ u_q(x)
\quad\text{s.t.\ per-prompt or pooled budgets}
\qquad=\qquad
\max_{\Phi}\ \min_{\varpi\in\Simp(\X)}\ \E_{x\sim\varpi}\big[u_q(x)\big].
\tag{C}
\end{equation}
The equality rewrites the worst prompt as the worst mixture (the inner objective is linear
in $\varpi$, so its minimum is attained at a vertex); $\min_\varpi$ over all of
$\Simp(\X)$ is the distributionally robust objective with the largest ambiguity set, and
any smaller set $\mathcal K\ni\Dist$ interpolates between \eqref{eq:B}
($\mathcal K=\{\Dist\}$) and \eqref{eq:C}.

\begin{remark}[The optimum is a \emph{rule}, computed in two stages]
\label{rem:two-stage}
It is tempting to read ``averaging over $x$'' in \eqref{eq:B} as eliminating the prompt
from the solution. It does not. Pooling eliminates $x$ from the \emph{constraints} and from
the scalar objective, but the decision variable is the whole decoder
$\Phi:x\mapsto q(\cdot\mid x)$, and the optimum is a rule, not a single distribution.
Equivalently: $(T,\eta)$ is a global \emph{operator} and
$\big(p(\cdot\mid x),U(\cdot,x)\big)$ is its prompt-local \emph{argument}. At fixed global
multipliers the Lagrangian integrand at prompt $x$ depends only on $q(\cdot\mid x)$, so the
inner maximization is pointwise and its argmax responds to the local pair even though the
multipliers do not. Pooling flattens the operator, never the argument; the only way
$\qst(\cdot\mid x)$ could be $x$-free is the degenerate case in which
$p(\cdot\mid x),U(\cdot,x)$ are constant in $x$. (Compare cross-validated ridge: the
penalty is chosen from the data distribution with no test point in hand; the prediction
still depends on the realized $x$.)

The two stages are therefore: \emph{design} (offline, $x$ random and only $\Dist$ known)
solves the two budget equations for the scalars $(T,\eta)$ from a calibration sample of
$\Dist$ alone; \emph{inference} (online, $x$ realized) runs the backward sweep of Lemma~1
on $\big(p(\cdot\mid x),U(\cdot,x)\big)$ at those prices to obtain $V^{\,x}$, then
samples \eqref{eq:tilt}. Since $V$ depends on the prices as well as on the prompt, the
sweep in \eqref{eq:B} uses the same global $(\lamst,\must)$ at every prompt, whereas in
\eqref{eq:A} each prompt's sweep uses its own.
\end{remark}

\begin{theorem}[Invariance]
\label{thm:inv}
Assume $\lambda^\star > 0$ and $\mu^\star > 0$. In each of \eqref{eq:A}, \eqref{eq:B}, \eqref{eq:C} the optimal
decoder is, at every $x$, prefix $w^{t-1}$ and token $w$,
\begin{equation}\label{eq:tilt}
\qst_t(w\mid w^{t-1},x)
=\frac{\big(p_t(w\mid w^{t-1},x)\,\exp\!\big(\eta\,V^{\,x}_t(w\mid w^{t-1})\big)\big)^{1/T}}
{Z_t(w^{t-1},x;T,\eta)},
\end{equation}
the tilted-temperature family of Theorem~1 applied prompt-wise, with $V^{\,x}$ the
potential of Lemma~1 for the pair $\big(p(\cdot\mid x),U(\cdot,x)\big)$ at the prices in
force. The formulations differ only in how $(T,\eta)$ are pinned:
\begin{itemize}[leftmargin=2.2em,itemsep=2pt]
\item[(A)] $(T,\eta)=\big(T(x),\eta(x)\big)$, solving the two budget equations
$\Hbar_q(x)=\beta(x)$, $\CE_q(x)=\gamma(x)$ separately at each prompt; the potential
$V^{\,x}$ is built at that prompt's prices.
\item[(B)] $(T,\eta)$ is a single global pair, solving the two pooled budget equations
$\E_\Dist[\Hbar_q]=\beta$, $\E_\Dist[\CE_q]=\gamma$; every $V^{\,x}$ is built at those
global prices.
\item[(C)] \emph{Per-prompt budgets:} \eqref{eq:C} is solved by the optimum of
\eqref{eq:A}, and robustness is vacuous. \emph{Pooled budgets:} $(T,\eta)$ is the single
global pair pinned by the two budget equations evaluated under a least-favorable mixture
$\varpi^\star\in\Simp(\X)$, and $\qst$ equalizes the per-prompt success on its support,
$u_{\qst}(x)=\min_{x'}u_{\qst}(x')$ for all $x\in\operatorname{supp}\varpi^\star$.
\end{itemize}
\end{theorem}

\begin{proof}
Throughout, write the per-prompt Lagrangian integrand at prices $(\lambda,\mu_E)$,
\begin{equation}\label{eq:Lx}
\mathcal L_x\big(q(\cdot\mid x)\big)
:= u_q(x)+\sum_{t=1}^{n}\E_{w^{t-1}\sim q}\Big[\tfrac{\mu_E}{n}H(q_t)
+\lambda\textstyle\sum_w q_t\log p_t\Big],
\end{equation}
which is exactly the objective appearing in the proof of Theorem~1 for the fixed prompt
$x$: a finite-horizon control problem with terminal reward $U(\cdot,x)$ and per-step reward
$\lambda\E_{q_t}[\log p_t]+\tfrac{\mu_E}{n}H(q_t)$. By that proof --- Lemma~2 applied node
by node to the optimal cost-to-go --- its unique maximizer is \eqref{eq:tilt} with
\begin{equation}\label{eq:prices}
\lamst=\frac{n\lambda}{\mu_E},\qquad \must=\frac{n}{\mu_E},\qquad
T=\frac{1}{\lamst}=\frac{\mu_E}{n\lambda},\qquad \eta=\frac{\must}{\lamst}=\frac1\lambda ,
\end{equation}
and $V^{\,x}$ the Lemma~1 potential of $\big(p(\cdot\mid x),U(\cdot,x)\big)$ at
$(\lamst,\must)$: it is the optimal cost-to-go itself,
$V^{\,x}_t(w\mid w^{t-1})=J_{t+1}(w^{t-1}w)$, produced by the dynamic program and
depending on no policy. Also, in occupancy-measure coordinates $u_q(x)$ and $\CE_q(x)$ are
linear and $\Hbar_q(x)$ is concave, so each per-prompt program is convex on a convex compact
set, and Slater's condition holds whenever $\beta<\log|\W|$ and $\gamma$ is not
binding-tight.

\smallskip
\noindent\emph{(A).} Objective and constraints are both collections of per-prompt terms,
and every term at $x$ involves only $q(\cdot\mid x)$. Hence \eqref{eq:A} separates into
independent copies of (PE), one per $x$; each is solved by Theorem~1, whose duals
$(\lamst(x),\must(x))$ --- and hence
$\big(T(x),\eta(x)\big)=\big(1/\lamst(x),\must(x)/\lamst(x)\big)$ --- are pinned by that
prompt's two active constraints.

\smallskip
\noindent\emph{(B).} Introduce scalar multipliers $\mu_E\ge0$ (pooled entropy floor) and
$\lambda\ge0$ (pooled cross-entropy ceiling). The Lagrangian is
\[
\mathcal L(\Phi;\lambda,\mu_E)=\E_{x\sim\Dist}\big[\mathcal L_x(q(\cdot\mid x))\big]-\mu_E\beta+\lambda\gamma .
\]
At fixed $(\lambda,\mu_E)$ the expectation is of terms each depending on a single
restriction $q(\cdot\mid x)$, so $\max_\Phi\mathcal L$ decouples across prompts,
$\max_\Phi\E_x[\mathcal L_x]=\E_x[\max_{q(\cdot\mid x)}\mathcal L_x]$, the pointwise
maximizers being measurable in $x$ by \eqref{eq:tilt} (a continuous function of the
conditionals and of $V^{\,x}$, itself a continuous function of the conditionals through
$n$ log-sum-exps). Each inner problem is \eqref{eq:Lx}, so its solution is \eqref{eq:tilt}
with the prices \eqref{eq:prices} --- \emph{global}, because $(\lambda,\mu_E)$ are global,
while the tilted object $\big(p(\cdot\mid x),V^{\,x}\big)$ is local. Convexity plus
Slater gives strong duality, so the maximizer of $\mathcal L$ at the optimal multipliers
solves \eqref{eq:B}, and $(\lambda,\mu_E)$ are fixed by complementary slackness at the two
pooled active constraints $\E_\Dist[\Hbar_q]=\beta$, $\E_\Dist[\CE_q]=\gamma$.

\smallskip
\noindent\emph{(C), per-prompt budgets.} In \eqref{eq:A} both the objective and the
constraints separate, so its optimum maximizes $u_q(x)$ \emph{pointwise}, subject to that
prompt's budgets. A decoder that maximizes every $u_q(x)$ simultaneously maximizes
$\min_x u_q(x)$ as well; hence the \eqref{eq:A}-optimum solves \eqref{eq:C} and nothing is
lost by ignoring the robust objective. Prompts do not compete: each has its own budget.

\smallskip
\noindent\emph{(C), pooled budgets.} Now prompts compete for one budget and the problem is
a genuine saddle point. Pass to occupancy-measure (causal) coordinates: a decoder is
equivalent to a causal visitation $\omega=(\omega_x)_{x\in\X}$, in which
$u_q(x)=\langle\omega_x,U_x\rangle$ is linear in $\omega$, the pooled cross-entropy is
linear, and the pooled causal entropy is concave; the feasible set $\Omega$ is therefore
convex and compact. The rewritten objective
\[
G(\omega,\varpi):=\sum_{x}\varpi(x)\,\langle\omega_x,U_x\rangle
\]
is bilinear: linear (hence concave) in $\omega$ on $\Omega$, and linear --- hence convex and
continuous --- in $\varpi$ on the compact simplex $\Simp(\X)$. Sion's minimax theorem
applies, so $\max_\omega\min_\varpi G=\min_\varpi\max_\omega G$ and a saddle point
$(\omega^\star,\varpi^\star)$ exists. For fixed $\varpi$, the inner
$\max_\omega G(\cdot,\varpi)$ is exactly formulation \eqref{eq:B} with $\Dist$ replaced by
$\varpi$; hence its solution is \eqref{eq:tilt} with the \emph{single global} pair
$(T,\eta)$ pinned by the budgets under $\varpi$. Evaluating at $\varpi^\star$ gives the
stated form. Finally, optimality of $\varpi^\star$ in the outer min is a linear program
over $\Simp(\X)$ with cost $u_{\qst}(x)$; its optimal support lies in
$\argmin_x u_{\qst}(x)$, and complementary slackness forces $u_{\qst}(\cdot)$ to be constant
$\big(=\min_{x'}u_{\qst}(x')\big)$ on $\operatorname{supp}\varpi^\star$ --- the
equalization claim.
\end{proof}


==> proofProp1.tex <==
\section{How to choose $\beta$} 
\label{app:beta}

\noindent\textbf{Where $k$ enters the decoder.}
Since $\passk(q)=1-(1-u_q)^k$ is strictly increasing in $u_q$, for any fixed budgets $(\beta,\gamma)$ the maximizer of (PE) is the single tilted-temperature policy of Theorem~\ref{thm:tilt} and is \emph{independent of $k$}. The sample budget therefore enters the decoder only through the choice of entropy floor $\beta$: ``larger $k$ wants hotter'' is not a property of the optimal decoder at a fixed operating point, but of how the diversity budget is spent as $k$ grows. Making that dependence explicit requires an exogenous rule for selecting $\beta$ as a function of $k$; a natural one maximizes $\passk$ regularized by a strictly convex, strictly decreasing diversity-cost $S$,
\[
\beta^\star(k):=\argmax_{\beta\in[0,\log|\W|]}\ \big\{1-(1-u(\beta))^k-S(\beta)\big\},\qquad\text{e.g. } S(\beta)=c\,(\log|\W|-\beta)^2 ,
\]
where $u(\beta)$ is the optimal success at floor $\beta$ and $\lambda^\star(\beta)$ the corresponding cross-entropy dual. Under this rule larger $k$ favors a higher floor but,  as one should expect from the non-monotonicity of the pass@$k$ sensitivity $\sigma_k$ (Theorem~\ref{thm:partial}(iii)), only once the operating point is in the high-coverage regime; below it the comparative static reverses. The result below records this; note that $S$ is a modeling choice, so the statement concerns the induced budget schedule, not the optimum of (PE) itself. 

\begin{proposition}[Budget-selection comparative static]\label{prop:mono}
Assume $u:[0,\log|\W|]\to(0,1)$ is $C^1$ and strictly decreasing, $S$ is $C^1$, strictly decreasing and strictly convex, the dual $\lambda^\star(\beta)>0$ is non-increasing in $\beta$ on the budget range under consideration, and each $\beta^\star(k)$ is a non-degenerate interior maximizer. Then at every such $k$,
\[
\operatorname{sign}\tfrac{d}{dk}\beta^\star(k)=\operatorname{sign}\big(\passk(\beta^\star(k))-(1-e^{-1})\big).
\]
Consequently, on any budget range where the operating point clears the coverage line $\passk(\beta^\star(k))\ge 1-e^{-1}$ (equivalently $(1-u(\beta^\star(k)))^k\le e^{-1}$), the floor $\beta^\star(k)$---and hence the induced temperature $T^\star(k):=1/\lambda^\star(\beta^\star(k))$---is non-decreasing, strictly at interior points where the inequality is strict; below the crossover $k_0=-1/\log(1-u^\star)\approx 1/u^\star$ it is non-increasing. Since $\beta^\star(k)\to\log|\W|$ and $\passk(\beta^\star(k))\to1$ as $k\to\infty$, all sufficiently large $k$ lie in the increasing regime.
\end{proposition}

We prove Proposition~\ref{prop:mono} next. But first we recall the budget-selection objective
\[
G_k(\beta):=\underbrace{1-(1-u(\beta))^k}_{=:F_k(\beta)}-S(\beta),
\qquad
\beta^\star(k):=\argmax_{\beta\in[0,\log|\W|]}G_k(\beta),
\]
with $u:[0,\log|\W|]\to(0,1)$ the optimal success at floor $\beta$ ($C^1$, strictly
decreasing), $S$ the $C^1$, strictly decreasing, strictly convex diversity cost, and
$T^\star(k)=1/\lambda^\star(\beta^\star(k))$ with $\lambda^\star(\cdot)>0$
non-increasing on the budget range under consideration. It is convenient to write $v(\beta):=1-u(\beta)\in(0,1)$, so $v$ is
strictly increasing with $v'(\beta)=-u'(\beta)>0$. We treat the budget $k\ge1$ as a
continuous parameter; the integer statement follows by restriction, and a discrete
cross-check. Figure~\ref{fig:tstar} illustrates the comparative static
synthetically and on a real language model.
\begin{figure}[!htbp]
\centering

\begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_Tstar_k.pdf}
    \caption{Synthetic illustration.}
    \label{fig:tstar-synth}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{empirical_Tstar_vs_k_humaneval_red.pdf}
    \caption{Empirical HumanEval sweep.}
    \label{fig:tstar-human}
\end{subfigure}

\caption{\textbf{Temperature as a function of sample budget.}
\textbf{(a)} For a synthetic instance, we select the entropy-floor point
maximizing pass@$k$ under the diversity cost $S$ and report the induced
temperature $T^\star(k)$.
\textbf{(b)} On 50 HumanEval problems with Qwen2.5-Coder-1.5B, we select the
best fixed temperature from $T\in[0.4,1.2]$ for each sample budget.
Both show the non-decreasing temperature--budget relation predicted by
Proposition~\ref{prop:mono}.}
\label{fig:tstar}
\end{figure}

\paragraph{The exact comparative static.}
Both derivatives below are elementary:
\begin{equation}\label{eq:app-Fk}
F_k'(\beta)=-k\,v(\beta)^{k-1}v'(\beta)<0,
\qquad
\partial_k F_k'(\beta)=-v'(\beta)\,v(\beta)^{k-1}\big(1+k\ln v(\beta)\big).
\end{equation}
The first shows $F_k$ is strictly decreasing in $\beta$ (a higher entropy floor
lowers coverage); the second is obtained by differentiating
$k\,v^{k-1}=k\,e^{(k-1)\ln v}$ in $k$.

\begin{lemma}[Sign of the comparative static]\label{lem:app-sign}
At a non-degenerate interior maximiser $\beta^\star(k)$ (i.e.\
$G_k'(\beta^\star)=0$ and $G_k''(\beta^\star)<0$), the selection $\beta^\star(\cdot)$
is $C^1$ near $k$ and
\[
\operatorname{sign}\frac{d\beta^\star}{dk}
=\operatorname{sign}\big(\partial_k F_k'(\beta^\star)\big)
=\operatorname{sign}\big(k(-\ln v^\star)-1\big)
=\operatorname{sign}\big(\passk(\beta^\star)-(1-e^{-1})\big),
\qquad v^\star:=1-u(\beta^\star(k)).
\]
\end{lemma}

\begin{proof}
Write the stationarity map $\Phi(\beta,k):=\partial_\beta G_k(\beta)=F_k'(\beta)-S'(\beta)$.
By hypothesis $\Phi(\beta^\star,k)=0$ and
$\partial_\beta\Phi(\beta^\star,k)=G_k''(\beta^\star)<0\neq0$, so the implicit
function theorem gives a $C^1$ selection $\beta^\star(\cdot)$ with
\[
\frac{d\beta^\star}{dk}
=-\frac{\partial_k\Phi(\beta^\star,k)}{\partial_\beta\Phi(\beta^\star,k)}
=-\frac{\partial_k F_k'(\beta^\star)}{G_k''(\beta^\star)},
\]
where $\partial_k\Phi=\partial_k F_k'$ because $S$ is $k$-free. As
$G_k''(\beta^\star)<0$, the sign equals that of $\partial_k F_k'(\beta^\star)$. By
\eqref{eq:app-Fk}, and since $v'>0$, $v^{k-1}>0$,
\[
\operatorname{sign}\big(\partial_k F_k'(\beta^\star)\big)
=\operatorname{sign}\big(-(1+k\ln v^\star)\big)
=\operatorname{sign}\big(k(-\ln v^\star)-1\big).
\]
Finally $k(-\ln v^\star)-1>0\iff (v^\star)^k<e^{-1}\iff
\passk(\beta^\star)=1-(v^\star)^k>1-e^{-1}$.
\end{proof}
\begin{corollary}[Hotter sampling for larger $k$]\label{prop:app-mono}
Under the stated regularity, on any budget interval $\mathcal K$ on which the optimal
operating point clears the coverage line,
\[
\passk\big(\beta^\star(k)\big)\ \ge\ 1-e^{-1}
\qquad\Longleftrightarrow\qquad
\big(1-u(\beta^\star(k))\big)^k\le e^{-1}
\qquad(k\in\mathcal K),
\]
the floor $\beta^\star(k)$ is non-decreasing on $\mathcal K$, strictly at every
interior $k$ where the inequality is strict; consequently
$T^\star(k)=1/\lambda^\star(\beta^\star(k))$ is non-decreasing on $\mathcal K$,
strictly at those $k$. Moreover this regime always obtains for all sufficiently
large $k$: $\beta^\star(k)\to\log|\W|$ and $\passk(\beta^\star(k))\to1$ as
$k\to\infty$.
\end{corollary}

\begin{proof}
On $\mathcal K$ the coverage inequality is exactly $(v^\star)^k\le e^{-1}$, i.e.\
$k(-\ln v^\star)-1\ge0$, so Lemma~\ref{lem:app-sign} gives
$\frac{d}{dk}\beta^\star(k)\ge0$ there, with strict inequality where
$(v^\star)^k<e^{-1}$. Integrating the $C^1$ selection over $\mathcal K$,
$\beta^\star$ is non-decreasing (strict at interior strict points). Since
$\lambda^\star(\cdot)$ is non-increasing, $\beta\mapsto1/\lambda^\star(\beta)$ is
non-decreasing, and composing with the non-decreasing $\beta^\star(\cdot)$ gives the
claim for $T^\star$.

For the large-$k$ statement, fix any $\beta_0<\log|\W|$. Because $u>0$ on
$[0,\log|\W|]$, $\min_{[\beta_0,\log|\W|]}u=:u_0>0$ and hence
$F_k(\beta)=1-(1-u(\beta))^k\to1$ uniformly on $[\beta_0,\log|\W|]$. Thus
$G_k\to1-S$ uniformly there, and since $S$ is strictly decreasing its maximiser over
$[\beta_0,\log|\W|]$ is $\log|\W|$; as $\beta_0$ is arbitrary,
$\beta^\star(k)\to\log|\W|$. Then $u(\beta^\star(k))\to u(\log|\W|)>0$, so
$\passk(\beta^\star(k))=1-(1-u(\beta^\star(k)))^k\to1\ge1-e^{-1}$, placing all large
$k$ in the regime.
\end{proof}

\begin{remark}[Where the naive global claim fails, and why it is expected]\label{rem:app-reverse}
Below the coverage line the comparative static \emph{reverses}: by
Lemma~\ref{lem:app-sign}, $\frac{d}{dk}\beta^\star(k)<0$ whenever
$\passk(\beta^\star(k))<1-e^{-1}$. The crossover budget is
\[
k_0(u^\star)=\frac{1}{-\ln(1-u^\star)}\ \approx\ \frac{1}{u^\star}\quad(u^\star\to0),
\]
which is exactly the maximiser of the pass@$k$ sensitivity
$\sigma_k=k(1-u)^{k-1}$ appearing in Theorem~\ref{thm:partial}(iii). At a base success rate
$u^\star\approx0.2$ one has $k_0\approx4.5$, so at $k=1,\dots,4$ the optimal floor
can \emph{decrease} in $k$ before the monotone regime takes over at $k\gtrsim5$; a
grid search over the quadratic cost $S(\beta)=c(\log|\W|-\beta)^2$ reproduces this
reversal precisely at the $1-e^{-1}$ threshold. The non-monotonicity is therefore
not a defect of the selection rule but the same low-coverage effect the paper
already isolates for $\sigma_k$; the folklore ``larger $k$ wants hotter'' is a
theorem precisely on the high-coverage side of $k_0$.
\end{remark}
\paragraph{Choosing the budgets $\beta$ and $\gamma$.}
The two budgets decouple, which makes them easy to set in practice. The
plausibility ceiling $\gamma$ fixes the \emph{temperature scale}: on the
tempered family $q_a\propto p^{a}$ the per-token cross-entropy
$\mathrm{CE}(q_a,p)$ is strictly monotone in the exponent $a=1/T$
(proof of Theorem~\ref{thm:collapse}), so $\gamma\leftrightarrow T$ is a
bijection. We therefore anchor $\gamma$ at a reference temperature $T_0$
trusted for the model and domain, $\gamma:=\mathrm{CE}(q_{1/T_0},p)$, computed
with a single forward pass over the calibration set and no sampling; $\gamma$
then reads as ``$q$ may drift from $p$ by at most the per-token cross-entropy
$T_0$ induces,'' and is loosened to explore or tightened for precision. The
entropy floor $\beta$ fixes \emph{diversity} and carries the budget dependence:
following Proposition~\ref{prop:mono}, we set
$\beta^\star(k)=\arg\max_{\beta\in[0,\log|W|]}\{\,1-(1-u(\beta))^k-S(\beta)\,\}$
with a strictly convex, decreasing diversity cost $S(\beta)=c(\log|W|-\beta)^2$,
whose maximizer is non-decreasing in $k$ on the high-coverage regime---cold
floors for small $k$, hot floors for large $k$. The single constant $c$ trades
coverage against diversity and is fixed once per domain on validation pass@$k$;
absent an optimization, any schedule rising from $H(p)$ toward $\log|W|$
reproduces the same behavior. Feasibility requires only joint attainability:
the base model realizes $(\beta,\gamma)=(H(p),H(p))$, so any $\beta\le H(p)$
with $\gamma\ge H(p)$ admits $q=p$, and driving $\beta$ above $H(p)$ demands a
$\gamma$ loose enough to license the hotter optimum. Both quantities are
occupancy-weighted per-token averages, hence estimated from a handful of
calibration prompts at one forward pass each---exactly what CTD's Phase~1 computes.


==> proofTh1.tex <==
\section{Full proof of Theorem~\ref{thm:tilt}}\label{app:proofTh1}
 Here we give it in full, in
particular the passage from the Lagrangian to the per-step cost-to-go the recursion (\ref{eq:app-J}) below, which is the principle of optimality specialised to the
entropy-regularised program \eqref{eq:PE}, and the strong-duality step that
certifies the resulting stationary point as the constrained optimum.

Throughout, a policy is $q=(q_1,\dots,q_n)$ with
$q(w^n)=\prod_{t=1}^n q_t(w_t\mid w^{t-1})$, and
$q(w^{t-1}):=\prod_{s<t} q_s(w_s\mid w^{s-1})$ is the occupancy of the prefix
$w^{t-1}$ induced by $q$. We write $\langle q_t,c\rangle:=\sum_w q_t(w)c(w)$.

\subsection{Step 0: Lagrangian relaxation}

Since $\passk(q)=1-(1-u_q)^k$ is strictly increasing in $u_q:=\E_{w^n\sim q}[U(w^n)]$,
program \eqref{eq:PE} is equivalent to maximising $u_q$ under the same two
constraints. Attach multipliers $\mu_E\ge0$ to the entropy floor
$\frac1n\sum_t\E_{w^{t-1}\sim q}[H(q_t)]\ge\beta$ and $\lambda_0\ge0$ to the
plausibility ceiling $-\frac1n\sum_t\E_{w^{t-1}\sim q}[\sum_w q_t\log p_t]\le\gamma$.
The Lagrangian is
\[
\mathcal L_0(q)
= u_q
+\mu_E\Big(\tfrac1n\textstyle\sum_t\E[H(q_t)]-\beta\Big)
-\lambda_0\Big(-\tfrac1n\textstyle\sum_t\E[\sum_w q_t\log p_t]-\gamma\Big).
\]
Dropping the additive constant $-\mu_E\beta+\lambda_0\gamma$ (which does not affect
the maximiser in $q$) and renaming $\lambda:=\lambda_0/n$,
\begin{align}\label{eq:app-lag}
\mathcal L(q)=&E_{w^n\sim q}[U(w^n)]
+\sum_{t=1}^n\E_{w^{t-1}\sim q}\big[\rho_t(w^{t-1},q_t)\big],\\
\rho_t(w^{t-1},q_t):=&\tfrac{\mu_E}{n}H\big(q_t(\cdot\mid w^{t-1})\big)
+\lambda\!\sum_w q_t(w\mid w^{t-1})\log p_t(w\mid w^{t-1}),
\end{align}
which is the Lagrangian displayed in the main text. It is a finite-horizon control
problem: terminal reward $U(w^n)$ at the leaves and per-step reward $\rho_t$, a
concave functional of the action distribution $q_t$. The $1/n$ rescaling is
``harmless'' in the precise sense that it only relabels the dual variable; the
optimal $\lambda$ recovered below is $1/n$ times the multiplier of the ceiling as
written in \eqref{eq:PE}.
It is illustrated in Figure~\ref{fig:proof-tree}.
\input{section_proof_tree2}

\subsection{Step 1: The recursion}

The one detail suppressed in the main text is why \eqref{eq:app-lag} collapses to a
node-wise recursion. This is the principle of optimality; we prove it for the
present objective, whose per-step ``reward'' is a functional of the whole
conditional $q_t$ rather than of a sampled action.

\begin{lemma}[Principle of optimality]\label{lem:app-poo}
Let $J_{n+1}(w^n):=U(w^n)$ and, for $t=n,n-1,\dots,1$ and every prefix
$w^{t-1}$,
\begin{equation}\label{eq:app-J}
J_t(w^{t-1}):=\max_{q_t\in\Delta(\W)}
\Big\{\rho_t(w^{t-1},q_t)+\sum_{w\in\W}q_t(w\mid w^{t-1})\,J_{t+1}(w^{t-1}w)\Big\}.
\end{equation}
Then $\max_q\mathcal L(q)=J_1(\varnothing)$, and any policy that attains the maximum
in \eqref{eq:app-J} at every node is a global maximiser of \eqref{eq:app-lag}.
\end{lemma}

\begin{proof}
For a fixed policy $q$ and a prefix $w^{t-1}$, let
\[
G^q_t(w^{t-1}):=
\E_{w_{t:n}\sim q}\Big[U(w^n)+\sum_{s=t}^n\rho_s(w^{s-1},q_s)\ \Big|\ w^{t-1}\Big],
\qquad G^q_{n+1}(w^n):=U(w^n),
\]
the conditional tail objective, the expectation being over $w_t,\dots,w_n$ drawn
from $q_t,\dots,q_n$ started at $w^{t-1}$. By the tower property applied to
\eqref{eq:app-lag}, $\mathcal L(q)=G^q_1(\varnothing)$. We show
$J_t(w^{t-1})=\max_{q_t,\dots,q_n}G^q_t(w^{t-1})$ by downward induction on $t$; the
case $t=1$ is the assertion.

\emph{Base.} $G^q_{n+1}=U=J_{n+1}$, with no maximisation.

\emph{Step.} Assume the claim at $t+1$ and fix $w^{t-1}$. The summand $\rho_t$ is
determined by $q_t$ given the prefix, so conditioning on the next token $w_t=w$ and
using the tower property,
\begin{equation}\label{eq:app-tower}
G^q_t(w^{t-1})=\rho_t(w^{t-1},q_t)+\sum_{w\in\W}q_t(w\mid w^{t-1})\,
G^q_{t+1}(w^{t-1}w).
\end{equation}
For each $w$ the term $G^q_{t+1}(w^{t-1}w)$ depends only on the conditionals
$(q_{t+1},\dots,q_n)$ restricted to the sub-tree rooted at $w^{t-1}w$, and these
sub-trees are pairwise disjoint across distinct $w$. Hence the tail conditionals may
be optimised independently within each sub-tree, and the coefficients
$q_t(w\mid w^{t-1})\ge0$ in \eqref{eq:app-tower} do not couple them:
\begin{align*}
\max_{q_t,\dots,q_n}G^q_t(w^{t-1})
=&\max_{q_t}\Big\{\rho_t(w^{t-1},q_t)
+\sum_w q_t(w\mid w^{t-1})\max_{q_{t+1:n}}G^q_{t+1}(w^{t-1}w)\Big\}\\
=&\max_{q_t}\Big\{\rho_t+\sum_w q_t\,J_{t+1}(w^{t-1}w)\Big\}
=J_t(w^{t-1}),
\end{align*}
where the second equality is the induction hypothesis and the last is
\eqref{eq:app-J}. The interchange of $\max_{q_t}$ with the inner maxima is licit
because, once each $\max_{q_{t+1:n}}G^q_{t+1}(w^{t-1}w)=J_{t+1}(w^{t-1}w)$ is a
constant in $q_t$, the outer bracket is a function of $q_t$ alone. Assembling the
node maximisers into a policy yields a global maximiser.
\end{proof}

Substituting $\rho_t$ from \eqref{eq:app-lag} into \eqref{eq:app-J} writes the
recursion in the form used in the main text,
\[
J_t(w^{t-1})=\max_{q_t\in\Delta(\W)}
\sum_w q_t(w)\big[\lambda\log p_t(w\mid w^{t-1})+J_{t+1}(w^{t-1}w)\big]
+\tfrac{\mu_E}{n}H(q_t),
\qquad J_{n+1}=U.
\]


\subsection{Step 2: Per-node Gibbs solution}

The bracket
$c(w):=\lambda\log p_t(w\mid w^{t-1})+J_{t+1}(w^{t-1}w)$ does not involve $q_t$, and
$\rho_t=\langle q_t,\lambda\log p_t\rangle+\tfrac{\mu_E}{n}H(q_t)$, so the node
problem is $\max_{q_t}\{\langle q_t,c\rangle+\tau H(q_t)\}$ with $\tau=\mu_E/n>0$.
Lemma~\ref{lem:gibbs} (the Gibbs variational principle) applies verbatim and gives
\[
q^\star_t(w\mid w^{t-1})=\frac{e^{c(w)/\tau}}{\sum_{w'}e^{c(w')/\tau}},
\qquad
J_t(w^{t-1})=\tau\log\sum_w e^{c(w)/\tau}.
\]
Since $c(w)/\tau=\tfrac{n}{\mu_E}\lambda\log p_t(w\mid w^{t-1})
+\tfrac{n}{\mu_E}J_{t+1}(w^{t-1}w)=\lambda^\star\log p_t+\mu^\star J_{t+1}$ with
$\lambda^\star:=n\lambda/\mu_E$ and $\mu^\star:=n/\mu_E$ (so $\tau=1/\mu^\star$),
\begin{align}\label{eq:app-node}
q^\star_t(w\mid w^{t-1}) &\propto
p_t(w\mid w^{t-1})^{\lambda^\star}\exp\!\big(\mu^\star J_{t+1}(w^{t-1}w)\big),\\
J_t(w^{t-1})&=\tfrac{1}{\mu^\star}\log\sum_w
p_t(w\mid w^{t-1})^{\lambda^\star}\exp\!\big(\mu^\star J_{t+1}(w^{t-1}w)\big).
\label{eq:app-node2}
\end{align}

\subsection{Step 3: Identification with the potential of Lemma~\ref{lem:bellman}}

Set $V_t(w\mid w^{t-1}):=J_{t+1}(w^{t-1}w)$. The left identity in
\eqref{eq:app-node} is \eqref{eq:opt1}--\eqref{eq:opt2} with temperature
$T=1/\lambda^\star$ and tilt $\eta=\mu^\star/\lambda^\star$. The terminal value is
$V_n(w\mid w^{n-1})=J_{n+1}(w^{n-1}w)=U(w^{n-1}w)=U(w^n)$, and the identity in
\eqref{eq:app-node2}, rewritten through $V$, is
\[
\tfrac1{\mu^\star}\log Z_t(w^{t-1}),\qquad
Z_t(w^{t-1})=\sum_w p_t(w\mid w^{t-1})^{\lambda^\star}
\exp\!\big(\mu^\star V_t(w\mid w^{t-1})\big),
\]
i.e.\ the terminal condition and backward recursion of Lemma~\ref{lem:bellman}. That
recursion involves only $(p,U,\lambda^\star,\mu^\star)$ and no policy, so $V_t$ is
its potential: the optimum is one backward sweep for $V$ followed by the forward
policy \eqref{eq:opt2}, with no self-consistent pair $(q^\star,V^\star)$ to solve.

\subsection{Step 4: Convexity, Slater, strong duality, complementary slackness}

It remains to certify that the Lagrangian stationary point is the constrained
optimum and that the multipliers are the two active constraints. Pass to causal
occupancy-measure coordinates: a policy is equivalent to a state--action visitation
$d=(d_t)_t$, $d_t(w^{t-1},w):=q(w^{t-1})\,q_t(w\mid w^{t-1})$, subject to the linear
causal-consistency (Bellman-flow) constraints
$\sum_w d_t(w^{t-1},w)=\sum_{w'} d_{t-1}(w^{t-2},w')\,\mathbf 1[(w^{t-2},w')=w^{t-1}]$
and $d_t\ge0$; the feasible set $\mathcal D$ is a convex compact polytope. In these
coordinates:
\begin{itemize}
\item $u_q=\sum_{w^n}d_n(w^{n-1},w_n)\,U(w^n)$ and the plausibility functional
$\frac1n\sum_t\sum_{w^{t-1},w}d_t\log p_t$ are \emph{linear} in $d$;
\item the causal entropy
$\frac1n\sum_t\sum_{w^{t-1},w}d_t\log\frac{\sum_{w'}d_t(w^{t-1},w')}{d_t(w^{t-1},w)}$
is a sum of conditional entropies, each \emph{concave} in $d$.
\end{itemize}
Hence \eqref{eq:PE} maximises a linear objective over $\mathcal D$ under one concave
($\ge$) constraint and one linear ($\le$) constraint: a convex program on a convex
compact set. Slater's condition holds whenever $\beta<\log|\W|$ (the uniform policy
is strictly entropy-feasible) and $\gamma$ is not at its binding-tight extreme, so a
strictly feasible $d$ exists. Strong duality then applies: at the optimal multipliers
$(\lambda,\mu_E)$ the unconstrained maximiser of $\mathcal L$ --- which by Steps~1--3
is the tilted-temperature policy \eqref{eq:opt1}--\eqref{eq:opt2} --- solves
\eqref{eq:PE}. Complementary slackness gives
\[
\mu_E\bigl(\bar H(q^\star)-\beta\bigr)=0,
\qquad
\lambda\bigl(\gamma-\mathrm{CE}(q^\star,p)\bigr)=0.
\]
Thus a slack constraint has zero multiplier. In the interior case where both multipliers
are positive, both constraints hold with equality and pin $(\lambda,\mu_E)$---equivalently
$(T,\eta)$---through the budgets $(\beta,\gamma)$.
\qed
\paragraph{The optimum is a single backward sweep.}
By Lemma~\ref{lem:bellman}, the potential $V_t$ in \eqref{eq:opt2} depends only on
$(p,U,\lambda^\star,\mu^\star)$. Hence, for fixed dual prices, it is obtained by
a single backward sweep, after which the optimal forward policy is given directly
by \eqref{eq:opt2}; no policy--value fixed point is required.

\begin{corollary}[Free-energy decomposition]\label{cor:freeenergy}
For $t<n$, with $q^\star$ from \eqref{eq:opt2} and
$\mathrm{CE}(q,p):=-\sum_w q(w)\log p(w)$,
\[
V_t(w\mid w^{t-1})
=
\underbrace{
\E_{w'\sim q^\star_{t+1}(\cdot\mid w^{t-1}w)}
\!\big[V_{t+1}(w'\mid w^{t-1}w)\big]
}_{\text{expectation backup of }V}
+
\frac{1}{\mu^\star}
\Big[
H\big(q^\star_{t+1}\big)
-\lambda^\star\,\mathrm{CE}\big(q^\star_{t+1},p_{t+1}\big)
\Big].
\]
Thus $V_t$ is an expectation backup augmented by an entropy--plausibility
free-energy correction. Since
$\mathrm{CE}(q,p)=H(q)+\mathrm{KL}(q\Vert p)$, the correction can be written as
\[
\frac{1}{\mu^\star}
\Big[
(1-\lambda^\star)H\big(q^\star_{t+1}\big)
-\lambda^\star\mathrm{KL}\big(q^\star_{t+1}\Vert p_{t+1}\big)
\Big],
\]
so its sign is not fixed in general.
\end{corollary}
\vspace{-0.05in}
\begin{proof}
Take $\log$ of \eqref{eq:opt2} at step $t+1$ and average under
$q^\star_{t+1}$. Since
$\sum_{w'}q^\star_{t+1}\log q^\star_{t+1}=-H(q^\star_{t+1})$, we obtain
\[
-H(q^\star_{t+1})
=
-\lambda^\star\mathrm{CE}(q^\star_{t+1},p_{t+1})
+\mu^\star\E[V_{t+1}]
-\log Z_{t+1}.
\]
Solving for $\log Z_{t+1}$ and using
$V_t=\mu^{\star-1}\log Z_{t+1}$ from Lemma~\ref{lem:bellman} gives the claim.
\end{proof}


==> related.tex <==

\section{Expanded Related Work}
\label{app:related}

A recent line of work treats the number of samples drawn at decoding as a
resource to be scaled, in analogy with parameters and pretraining tokens.
\citet{brown2024monkeys} show that coverage---the fraction of problems solved
by \emph{any} of $k$ samples, i.e.\ $\mathrm{pass@}k$---grows log-linearly over
several orders of magnitude in $k$, and \citet{wu2024inference} chart the
compute-optimal frontier between model size and sample count.
\citet{snell2024scaling} make the allocation adaptive, spending more
inference compute on harder prompts. These studies establish
$\mathrm{pass@}k$ as the operational objective but treat the sampling
distribution as fixed (typically the base model at a hand-tuned temperature);
our contribution is to ask which decoding distribution \emph{maximizes}
$\mathrm{pass@}k$ under an explicit compute budget, and to show that the
answer is the tilted-temperature as in ~\eqref{eq:opt1}.

\textit{Verifiers and selection.}
A complementary thread improves the \emph{selection} step rather than the
proposal distribution. Outcome-level verifiers trained on solution
correctness \citep{cobbe2021gsm8k}, process reward models that score
intermediate steps \citep{lightman2024verify}, and best-of-$n$ reranking
against a learned reward \citep{nakano2021webgpt} all re-weight a fixed pool
of samples. Our verifier signal plays a different role: rather than being used only to
select among completed samples, it enters the proposal distribution through
the continuation potential. In \textsc{J-EOS}, this potential is estimated
from terminal verifier feedback, while under the calibration conditions of
Section~\ref{sec:calib} its effect can be absorbed into the tempered
sequence law. Self-consistency
\citep{wang2023selfconsistency} can be read as a verifier-free aggregator and
is recovered as a special case when the verifier is uninformative.

\textit{Temperature and truncation decoding.}
Heuristic decoding modifications---nucleus sampling
\citep{holtzman2020degeneration} and truncation-as-desmoothing
\citep{hewitt2022truncation}---reshape the next-token distribution to trade
diversity against quality. These transformations are justified empirically; we instead derive the
optimal reshaping from a constrained $\passk$ objective. Under perfect
calibration the optimum reduces to a pure power of the base sequence law,
and ordinary per-token temperature sampling closely approximates this
optimum when the remaining-horizon correction has limited variation across
candidate tokens at each prefix.

\textit{Tilted distributions and KL-regularized control.}
The optimum $q^\star\propto\bigl(p\,e^{\eta V}\bigr)^{1/T}$ is an
exponentially tilted (Gibbs) distribution, the same form that arises from the
maximum-entropy principle \citep{jaynes1957information,cover2006elements} and
from KL-regularized control. Casting decoding as inference in a soft-optimal
MDP \citep{ziebart2008maxent,levine2018rlinference} and viewing the KL penalty
in RLHF as Bayesian conditioning \citep{korbak2022rlbayesian} both produce
tilted policies; \citet{rafailov2023dpo} exploit the closed form of the tilt to
bypass explicit reward modeling. We share the tilted-distribution structure but
work at inference time under a cross-entropy (compute) budget rather than a
training-time KL penalty, which is what pins the temperature $T=1/\lambda^\star$
to the budget.

\textit{Calibration.}
Our reduction from verifier estimation to temperature rests on calibration of
the base model's log-probabilities. Temperature scaling and Platt scaling
\citep{platt1999probabilistic,guo2017calibration} are the standard
post-hoc calibrators we adopt for the affine model of Section~\ref{sec:calib}; calibration
of pretrained transformers \citep{desai2020calibration} and the finding that
language models are partly aware of their own correctness
\citep{kadavath2022know} motivate the $(s,\varepsilon)$-calibration assumption.
Theorem~\ref{thm:partial} quantifies how the residual
miscalibration $\varepsilon$ degrades $\passk$, and
Theorem~\ref{thm:ctd} the finite-sample cost of estimating
the calibration slope $s$.

\textbf{Literature on practical algorithms.} A separate line of work adapts the sampling rule online rather than fixing it in
advance. Mirostat \citep{basu2021mirostatneuraltextdecoding} targets a fixed
perplexity level, while locally typical sampling \citep{meister-etal-2023-locally}
and $\eta$-sampling \citep{hewitt2022truncation} truncate using token-level
information content or entropy. More recent methods adapt using confidence or
structure: AdapT \citep{zhu2024hot} raises sampling temperature at line-initial
tokens, while AdaDec \citep{he2026adadecuncertaintyguidedlookaheaddecoding}
combines an entropy threshold with lookahead reranking. Its final token selection
is deterministic, so repeated decoding adds no sampling diversity and pass@$k$
collapses to pass@$1$. ARGS \citep{ICLR2024_4d134431} similarly performs
reward-guided greedy selection, and Uncert-CoT
\citep{zhu2025uncertaintyguidedchainofthoughtcodegeneration} triggers multi-path
reasoning above an uncertainty threshold.

